Visual Interaction with Deep Learning Models through Collaborative Semantic Inference

Automation of tasks can have critical consequences when humans lose agency over decision processes. Deep learning models are particularly susceptible since current black-box approaches lack explainable reasoning. We argue that both the visual interface and model structure of deep learning systems need to take into account interaction design. We propose a framework of collaborative semantic inference (CSI) for the co-design of interactions and models to enable visual collaboration between humans and algorithms. The approach exposes the intermediate reasoning process of models which allows semantic interactions with the visual metaphors of a problem, which means that a user can both understand and control parts of the model reasoning process. We demonstrate the feasibility of CSI with a co-designed case study of a document summarization system.

==> Latvaria(IEEEVAST2019) (2)/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Latvaria(IEEEVAST2019) (2)/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> Latvaria(IEEEVAST2019) (2)/src/01-intro.tex <==
%% \section{Introduction} %for journal use above \firstsection{..} instead
Deep learning has become a universal tool that is increasingly applied in automated approaches to commonplace problems. 
Often, improvements in performance and efficiency from deep models come at the cost of increased model complexity, which leads to difficulties in interpretation, analysis, and visualization. 
By relying on the outputs of these complex black-box models, users give up their agency and control over the automated process. 
Moreover, the users are forced to trust and rely on models that have been shown to be biased, and that can make inexplicable mistakes.\looseness=-1

% This is too cute
%Recent examples how a loss of agency can lead to harmful effects are the crashes of multiple aircraft that have been partially attributed to the increasing automation of the cockpit~\cite{wise_2019,potocnik2018tragic}. 

To combine the advantages of models and humans, researchers across disciplines have advocated for models as collaborative team members. Grosz argues that the development of ``intelligent, problem-solving partners is an important goal in the science of AI''~\cite{grosz1996collaborative}. Horvitz' principles for mixed-initiative user interfaces~\cite{horvitz1999principles} and the more recent guidelines for human-AI interaction~\cite{amershi2019guidelines} call for ``mechanisms for efficient agent-user collaboration to refine results.'' 
Similarly, Heer points out that work on automation ignores the design space in which computational assistance augments and enriches people's intellectual work~\cite{Heer1844}.

We propose a framework that can be applied to enable users to control predictive processes called \emph{collaborative semantic inference} (CSI). CSI describes a dialogue, alternating between model predictions presented in a visual form and user feedback on internal model reasoning. 
This process requires exposing the model's internal process in a way that mirrors the \textit{users mental model} of the problem and then empowering the user to influence this process.
This approach is centered around the core design principles for visual analytics, which integrates visualization and analytics in a human-centered interface~\cite{keim2008visual}. 
Endert et al.~\cite{endert2012semantic} define semantic interactions as those which  ``enable analysts to spatially interact with [such] models directly within the visual metaphor using interactions that derive from their analytic process.''
CSI describes \textit{how} to connect these semantic interactions to the model inference process.
The development of CSI methods and interfaces further requires a tight collaboration between the visual analytics, interaction design, and machine learning experts, which is a challenging, but promising, direction of research~\cite{sacha2019vis4ml,endert2017state,stolper2014progressive,hohman2018visual}.

Most deep neural networks do not expose their internal reasoning process. The CSI framework requires the development of model extensions that expose intermediate reasoning that can be associated with user-understandable choices. In this work, we present a proposal that incorporates discrete latent variables~\cite{kim2018tutorial} into the model design. % EXAMPLE HERE? 
%\rk{short example would be helpful, otherwise difficult to understand at this point in the paper.}
These variables act as ``hooks'' that can control the reasoning process and output of a model. The hooks enable what-if analyses by answering what internal choices would have led to a specific output. Crucially for CSI, the hooks also allow a user to infer the model's reasoning process by seeing how a given output was selected. This visual analysis in the backward direction, from prediction to input, is typically not possible without model modifications.

To contextualize the multi-disciplinary co-design process and assist in developing collaborative tools, we provide an overview of the visualization and interaction design space for neural network models.
We describe the actions required to move towards the goal of retaining human agency through visual CSI interfaces. We further connect our categorization to the previously described user roles of architect, trainer, and end-user~\cite{strobelt2018lstmvis} and a classification into interpretability methods that aim to understand and shape the model or its decisions. 
%Our categorization classifies approaches as passive, or interactive observation approaches in the absence of feedback mechanisms that link back to the model and we describe methods to enable collaborative interactions for observation tools.

As proof of concept, we apply our design process to the use case of a document summarization system. When this task is handled by an automated system, the results almost always require heavy post-editing by humans. Our use-case presents a first attempt at a collaborative, deep learning-based, interface for this problem. This use-case also demonstrates the expanded design space of interactive visual interfaces for collaborative models. We further identify challenges encountered in these collaborative models: How do we develop an interface that visualizes the prediction process on a granular level for any kind of model-specific input type (e.g.,\ text, images, spectrograms), and how can a visual interface provide an integration of human interventions as part of the prediction process.

The paper contains the following contributions. In Section~\ref{sec:design}, we define the \textbf{concept of collaborative semantic inference} and its place in the design space of integrating deep neural models with visually interactive interfaces. We then describe \textbf{how CSI can be incorporated} into models using latent variables in Section~\ref{sec:latvar}. We \textbf{showcase a visually interactive use-case} for applying CSI to a text summarization task in Section~\ref{sec:uc2}. Based on our experience gained from this use case, we describe learned lessons towards building a systematic co-design process (Section~\ref{sec:process}). We discuss the implications of CSI and its advantages and disadvantages in Section~\ref{sec:conclusion}.

% The first contribution of this paper is an analysis of the design space for integrating models and a user interface, presented in Section~\ref{sec:design}. The second one is the development of the CSI model to develop interactive, collaborative interfaces, shown in Section~\ref{sec:latvar}. Our third contribution is the exploration of the described design space for the summarization problem and the design of a collaborative summarization interface in Section~\ref{sec:uc2}. Finally, we combine the lessons learned from this and related project into a process model which we describe in Section~\ref{sec:process}. We discuss the implications of CSI models and its advantages and disadvantages in Section~\ref{sec:disc}.


% \begin{itemize}
%     \item Contributions:
%     \item Design Space framework
%     \item Latent Variables as interpretable hooks
%     \item Use Cases
% \end{itemize}


%Automated and semi-automated approaches are becoming increasingly commonly applied to everyday problems. While automation can improve the efficiency of users of these algorithms, this is typically achieved at the cost of autonomy and agency. 

%As users lose their agency, it becomes crucial to provide an appropriate level of oversight of the algorithms to prevent model-intrinsic biases to discriminate against individuals affected by the model. 
%Thus, interpretability and transparency are necessary properties to be able to hold a model accountable for errors. Visualization and visual analytics help to address these challenges and are thus crucial parts of a machine learning pipeline to help understand the model training process, what a model has learned, and to debug errors.

%However, as models become increasingly complex and high-dimensional, they also grow more difficult to interpret, analyze, and visualize. 
%As deep learning continues to gain popularity, the extraction of meaningful information from trained models requires the development of appropriate analysis techniques at a similar pace. By developing the techniques only for already existing models, visual analytics is only an afterthought and as such always one step behind the modeling advances. Moreover, it presents the machine learning models as static entities that cannot be changed to accommodate improved visual analytics techniques that could improve the model interpretability. 
%To address this challenge, we propose an interaction framework in which visual interactions are a central aspect of the model design as part of a codesign process between machine learning and visual analytics researchers.

%Collaborative models are characterized through interpretable intermediate representations that can be utilized as targets for visual interactions. Moreover, collaborative models enable a bidirectional interaction between humans and the model such that the human can provide information for the model and vice versa. To fully utilize this interactive inference scheme for machine learning models, we further point out two visualization challenges: How to we develop an interface that visualizes the prediction process on a granular level for any kind of model-specific input type (e.g. text, images, spectrograms). Secondly, the interface needs to allow human interventions as part of the inference process.


==> Latvaria(IEEEVAST2019) (2)/src/02-design-space.tex <==
% \section{Design Space for Integrating Model and Visualization}
\section{Design Space for Integrating a Machine-Learned Model and Interactive Visualization}
\label{sec:design}

While previous work has categorized and described the vast design space for visual interpretation of machine learning models~\cite{endert2017state, liu2017towards, lu2017state, hohman2018visual}, the problem of co-designing models, visualizations, and interactions remains challenging. 
In an analysis, Crouser and Chang find that there exists no common language to describe human-computer collaboration interfaces in visual analytics and propose to reason about interfaces based on the possible interactions humans can have with a model~\cite{crouser2012affordance}.  

Expanding this idea, we contextualize different co-design approaches by categorizing the design space based on three criteria: (1) the level of integration of a machine learning model and a visually interactive interface, (2) the user type, and (3) applications that aim to understand and shape the model or model-decisions. Table~\ref{tab:cate} shows a categorization of the related work using criteria (1) and (3).

We identify three broad integration approaches between models and visual interfaces (Figure~\ref{fig:intmodel}): \emph{passive observations}, \emph{interactive observations}, and \emph{interactive collaborations}. 
As we will discuss in detail in this section, each category comprises a class of techniques that address different challenges of an analysis pipeline.
%The framework differentiates visualization techniques based on the type of possible interactions with a model, specifically to what extent a user can interact with the model and the model with the user. 

To decide on the visualizations and interactions for a specific problem in this design space we need to additionally consider the user type. We follow Strobelt et al.~\cite{strobelt2018lstmvis} who describe the roles of model \emph{architects}, \emph{trainers}, and \emph{end-users}. Architects are defined as users who are developing new machine learning methodologies or who adapt existing deep architectures for new domains. Trainers are those users who apply known architectures to tasks for which they are domain experts. 
End-users are those users who use trained models for various tasks and who may not know how a model functions. As domain experts, the end-users' main goal is to achieve and explain the results of a model.

% SG TODO: MAKE SUPER CLEAR THAT THIS IS ABOUT GOALS NOT CHOICES WHAT INTERACTIONS TO INCLUDE!
% Model-Understanding/Shaping: Systems with the goal of understanding or shaping the model through its features and parameters
%Decisions-Understanding/Shaping: Systems with the goal of understanding or shaping the individual decisions of the model on specific instances

In addition to the level of integration and user type, we divide the design space between visual interfaces to \emph{understand and shape the model or the decisions} of the model. 
Model-understanding/shaping describes systems with the goal of understanding or shaping the model through its features and parameters. The methods can help to gain insights into or modify the parameters that a model is in the process of learning or has learned already.
Decision-understanding/shaping systems have the goal of understanding or shaping the individual decisions of the model on specific instances. Decision-based applications aim to understand how the model arrives at a given output but does not modify the parameter of the model.
Shaping the model and decisions requires a tight coupling between the model and the interface, which in our classification is only possible with interactive collaboration interfaces, whereas the other categories focus on understanding. 

\begin{figure}[t!]
    \centering
    \includegraphics{"figs/CSI_user_interactions_monochrome"}
    \caption{We define the three levels of integration between models and visual interfaces: (a) passive observation, (b) interactive observation, and (c) interactive collaboration. Each successive stage extends the design space by adding new potential interactions. In the interactive collaboration stage, the model itself is extended with ``hooks'' to enable semantic interactions.}
    \label{fig:intmodel}
\end{figure}

\subsection{Passive Observation}

The first stage in our design space is passive observation, in which visualizations present a user with static information about the model or its output. The information can target any user-type and range from global information about model training to heatmaps overlaid over specific inputs. 
Passive observation interfaces only require a loose coupling between the interface and the model (Figure~\ref{fig:intmodel}(a)).

\paragraph{Model-Understanding}

Architects and trainers are often concerned about how well a model is training, i.e., the model \emph{performance}. 
Tools can assist trainers by tracking and comparing different models and metrics, e.g., Tensorboard~\cite{wongsuphasawat2018visualizing}.
Moreover, it is crucial for trainers to understand whether a model learns a good representation of the data as a secondary effect of the training, and to detect potential biases or origins of errors in a model~\cite{belinkov2019analysis}.
To address this issue, many model-understanding techniques aim to visualize or analyze learned global features of a model~\cite{zeiler2014visualizing,carter2019activation, odena2016deconvolution, belinkov2017neural}.
% An associated measure of evaluating a tool for this outcome is whether the monitoring leads do easier decisions about restarting or aborting training runs or whether the visualizations lead to a better mental model of the model performance.

\begin{table*}[t!]
\centering
\begin{tabular}{@{} >{\columncolor{white}[0pt][\tabcolsep]}p{.2\textwidth} %p{.16\textwidth} 
p{.35\textwidth} >{\columncolor{white}[\tabcolsep][0pt]}p{.35\textwidth} @{}}
\toprule
 & %Interaction with\dots& 
 Model-Understanding/Shaping & Decision-Understanding/Shaping  \\ \midrule
Passive Observation\newline
\textcolor{gray}{[Understanding]}& %Input & 
Activation Atlas~\cite{carter2019activation}, 
Classification Visualization~\cite{chae2017visualization},
DeepEyes~\cite{pezzotti2018deepeyes},
Feature classifiers~\cite{belinkov2017neural},
Tensorboard~\cite{wongsuphasawat2018visualizing},
Weight Visualization~\cite{tzeng2005opening} & 
Deconvolution~\cite{zeiler2014visualizing}, 
LIME~\cite{ribeiro2016should}, 
Neuron Analysis~\cite{dalvi2019one}, 
Rationals~\cite{lei2016rationalizing}, 
Saliency~\cite{li2015visualizing}, 
Structured Interpretation~\cite{dey2015predicting},
Prediction Difference~\cite{DBLP:conf/iclr/ZintgrafCAW17}\\ \addlinespace[0.2cm]
Interactive Observation\newline
\textcolor{gray}{[Understanding]} & %Input, Model Internals & 
ActiVis~\cite{kahng2018acti},
Deep Visualization~\cite{yosinski2015understanding}, 
Embedding Projector~\cite{smilkov2016embedding}, 
GANViz~\cite{wang2018ganviz}, 
LSTMVis~\cite{strobelt2018lstmvis}, 
Prospector~\cite{krause2016interacting}, 
RetainVis~\cite{kwon2019retainvis}, 
RNNVis~\cite{ming2017understanding}, 
ShapeShop~\cite{hohman2017shapeshop} & 
Instance-Level Explanations~\cite{krause2017workflow},
Manifold~\cite{zhang2019manifold}, 
NLIZE~\cite{liu2019nlize},
RNNBow~\cite{cashman2017rnnbow},
Semantic Image Synthesis~\cite{chen2017photographic}, 
Seq2Seq-Vis~\cite{strobelt2019s}\\
\addlinespace[0.2cm]
Interactive Collaboration\newline
\textcolor{gray}{[Shaping]} & %Input, Model Internals, Hooks, Output &
Human-in-the-Loop Training~\cite{holzinger2016interactive}, 
Statistical Active Learning~\cite{cohn1996active},
Tensorflow Playground~\cite{smilkov2017direct},
Explanatory Debugging~\cite{kulesza2010explanatory}
&
%\cellcolor{our_blue}
\textbf{Achievable via CSI}, for example in GANPaint~\cite{bau2018gandissect} \\ \bottomrule
\end{tabular}%
\vspace{1em}
\caption{A classification of some of the related work, which shows the distinct lack of collaborative interfaces for decision-understanding and shaping. Our CSI framework aims to fill this void, with a particular focus on applications built for end-users. However, different user types span all of the previous work, some aiming towards architects, trainers, end-users, or a combination of them.}
\label{tab:cate}
\end{table*}

\paragraph{Decision-Understanding}

Decision-understanding passive observation tools assist end-users in developing a mental model of the machine learning model behavior for particular examples. The most commonly applied decision-understanding techniques present overlays over images~\cite{ribeiro2016should,dey2015predicting} or texts~\cite{dalvi2019one,lei2016rationalizing,li2015visualizing}. These overlays often represent the activation levels of a neural network for a specific input. For example, in image captioning, this method can show a heatmap that indicates which part of an image was relevant to generate a specific word~\cite{DBLP:conf/icml/XuBKCCSZB15}. 
%It is challenging to define measures that accurately reflect whether the techniques achieve the desired outcome of developing a mental model of the behavior. 
A qualitative assessment of these methods may focus on whether highlights match human intuition before and after changes to the input or model~\cite{2017arXiv171100867K,SanityNIPS2018}. These methods also commonly assist in a pedagogical context~\cite{hohman2018visual,smilkov2017direct}. 

\subsection{Interactive Observation}

Interactive observation interfaces can receive feedback or information from the model itself (Figure~\ref{fig:intmodel}(b)). This feedback enables the testing of multiple hypotheses about the model behavior within a single interface.
We classify tools as interactive observation that allow changing inputs or extracting any model-internal representation as part of an interactive analysis. We call these \emph{forward} interactions, analogous to how sending inputs into a model is called the forward pass. This approach can be used by trainers with domain knowledge to verify that a model has learned known structures in the data, or by end-users to gain novel insights into a problem.
The development of interactive observation methods has been an active field of research, as summarized in recent review papers~\cite{liu2017towards, lu2017state, hohman2018visual}.
Interactive observation allows for a richer space of potential interactions than passive observation tools and thus require a closer coupling between visualizations, interface, and the model~\cite{endert2017state}.

\paragraph{Model-Understanding}

In an extension of visualization of learned features, interactive observational tools enable end-users and trainers to test hypotheses about global patterns that a model may have learned. One example is Prospector~\cite{krause2016interacting}, which can be used to investigate the importance of features and learned patterns.  Alternatively, counterfactual explanations can be used to investigate changes in the outcome of a model for different inputs, thereby increasing trust and interpretability~\cite{whatif,wachter2017counterfactual}.
%The visual approaches to integrate an expert's domain knowledge range from user-guided instance and feature selection.

\paragraph{Decision-Understanding}

Interactive decision-understanding tools visualize how minor changes to an input or the internal representation influences the model prediction. 
Interactively building this intuition is crucial to end-users since past research has shown that statically presenting only a few instances may lead to misrepresentation of the model limitations~\cite{kim2016examples} or the data that the model uses~\cite{vellido2012making}.
%The tool enables users to filter and then query the hidden states to find similar activations across the entire training set and overlays secondary properties on the results. 
Another desired outcome of interactive observational tools is the testing of hypotheses about local patterns that a model may have learned. For example, we developed Seq2seq-Vis~\cite{strobelt2019s}, which allows users to change inputs and constrain the inference of a translation model in order to pinpoint what part of the model is responsible for an error. This interaction is a type of non-collaborative shaping where the interactions are limited to the forward direction with the intended goal of understanding the decisions of the model.
Similar debugging-focused approaches~\cite{zhang2019manifold, krause2017workflow} only visualize the necessary parts of a model to find and explain errors, instead of giving in-depth insights into hidden model states.

%Due to the probabilistic nature of deep learning, defining quantitative measures for the outcomes is a challenging and unsolved problem. In our past work, we found it most helpful to run long-term studies and gather qualitative feedback instead. This enabled us to iteratively refine tools until the majority of the feedback confirmed the usefulness of the tool.

%\paragraph{Action} Instance-based passive observation techniques can be extended into interactive observations by including an interface for entering information or by precomputing the outcomes over a large set of data and providing a selection interface. For example, we developed LSTMVis to investigate whether active hidden states in a recurrent neural network are indicators of learned patterns~\cite{strobelt2018lstmvis}. While the tool does not allow evaluation of user-input, we precompute the states over the entire training set and enable search so that users can explore freely.


\subsection{Interactive Collaboration}

We characterize collaboration in interactive interfaces for deep learning models through the ability of end-users or trainers with domain knowledge to present feedback to the model (Figure~\ref{fig:intmodel}(c)) with the goal to shape the model or its decisions. We call these \emph{backward} interactions. 
Since each interaction direction needs to call a different shaping process within the model, the interface and model in interactive collaboration tools require a tight coupling. Only co-designing the model, visualizations, and interactions can achieve this tight integration. 

\paragraph{Model-Shaping}

On the model-level, the feedback is expressed as user-provided labels which can be used to change the model parameters in an active learning setting~\cite{holzinger2016interactive,cohn1996active,jiang2019recent}. 
In the forward direction, model performance can be visualized, and new samples for the labeling process can be selected \cite{holzinger2016interactive}. The model parameters can be updated through backward interactions~\cite{smilkov2017direct, kulesza2010explanatory}. 

\paragraph{Decision-Shaping} 

Interactive collaboration for decision-shaping requires an interface in which the end-user can guide the model-internal reasoning process to generate a different output than the model would have reached on its own. Since interactive collaborative interfaces also retain the ability for forward interactions, the intervention enables to an interplay between suggestions by the model and feedback by the user. Our proposed approach to developing CSI methods, which we describe in Section~\ref{sec:latvar}, presents one way to design such applications.\looseness=-1

% \paragraph{}
During forward interactions, the visualization shows what the model-internal reasoning process looks like for a specific input. During backward interactions, the end-user can modify the output and observe how the model-internal reasoning process would have looked like to arrive at that specific output. 
The incorporation of these feedback mechanisms into visual analytics tools requires three essential components. First, the model needs to expose an interpretable hook along its internal reasoning chain, which should be transparent in derivation and understandable for non-experts~\cite{lipton2016mythos}. Second, this interpretable hook needs to correspond to the mental model of the end-user. 
Most importantly, a collaborative tool needs to enable efficient interactions with the visual metaphor of the hook through semantic interaction~\cite{endert2012semantic}.  
%In this paper, we focus on describing interpretable hooks as latent variables within a model, a process that we describe in Section~\ref{sec:latvar}

%In addition, one can imagine the use of collaborative models as an extension of the user in a mixed-initiative user-inferface~\cite{horvitz1999principles} in use-cases where fully autonomous systems cannot be applied, for example in healthcare. Here, an associated measure is how the interface affects the efficiency and efficacy of the user compared to not using the tool.

The interpretable hooks of a model can act as explanations for rules of behavior that models learn. These explanations have been shown to improve model personalization~\cite{bostandjiev2012tasteweights} and explainability~\cite{caruana2015intelligible,kulesza2015principles}. Conversely, failing to provide explanations can inhibit the development of mental models in end-users~\cite{lim2009and}. However, explanations should also not overwhelm an end-user, and many previous approaches thus choose to select less complex models~\cite{lacave2002review} or aim to reduce the feature space of a trained model~\cite{craven1997using, yang1997comparative}.%\looseness=-1

CSI systems have models and end-users collaborate on the same output. This contrasts with previous work that often treats the model as a complementary assistant, for example recommending citations for a writer~\cite{babaian2002writer}.
Moreover, CSI argues for a design approach to collaborative interfaces where the user retains agency over the exposed parts of the model's reasoning process. 
Even in related approaches where the model and user both generate content, the users either do not have control over the model suggestions~\cite{guzdial2017general} or the model is replaced by uncontrollable crowdworkers~\cite{bernstein2010soylent}.
While previous work on interactive phrase-based machine translation showed promising results towards the goal of collaborative interfaces, the same techniques are not possible with deep learning-based approaches~\cite{green2014human}.
This lack of previous work (see Table~\ref{tab:cate}) can in part be attributed to the progress of deep learning methods, which have only recently reached the performance levels necessary for CSI-style interfaces. 

%Opposed to this, our proposed framework is agnostic to the model complexity, since the explanations are built into the model.

%\paragraph{Action} Collaborative interfaces require a codesign by both the model architect and the visualization expert. They have to decide on the desired interaction and the associated visual metaphor first. There are two possible model extensions that can be utilized for interactive collaboration models, and we will show one use-case for each approach in Sections~\ref{sec:uc1} and \ref{sec:uc2}. The first does not require any changes to the model itself but instead uses a second model to enable the backwards interaction. 

%Our first example is semantic image synthesis, where a user-defined input describes high-level features, for example the location of grass and sky, and a neural network generates the corresponding image~\cite{chen2017photographic, wang2018high, Park2019semantic}. However, the current approaches do not allow iterative refinement though interaction with an image. A collaborative approach to the same problem is GANPaint~\cite{bau2018gandissect}, which uses a second model to associate parts of the latent space of an image-generating model with the semantic features and exposes a modification interface to the user. 
%The second change, which we describe in Section~\ref{sec:latvar} aims to design discrete latent variables as a part of a model that correspond directly to the mental model of the user. These models are not explored within visual analytics tools, but there is active research in interpretable machine learning that aims to use latent variables as means to interpretability. For example, Hughes et al. develop a model for the classification of the correct antidepressant for a patient that constrains a set of latent variables to act as the explanation~\cite{hughes2018semi}. A visual interface for this model could enable the interaction with groups of these variables as an assistant to the doctor. 

==> Latvaria(IEEEVAST2019) (2)/src/03-related.tex <==
%\section{Related Work}

%Our framework combines insights from the fields of artificial intelligence, human-computer interaction, and visual analytics, some of which have a long-standing history. In the 1994 AAAI presidential address, Barbara Grosz argued that the development of ``intelligent, problem-solving partners is an important goal in the science of AI'' and that the capability of applications to collaborate with their users is ``essential''~\cite{grosz1996collaborative}. This call is further reflected in one of Horvitz' principles for mixed-initiative user interfaces~\cite{horvitz1999principles} and the more recent guidelines for human-AI interaction~\cite{amershi2019guidelines} which call for ``mechanisms for efficient agent-user collaboration to refine results.'' In a similar argument, Jeffrey Herr argues that work on automation does not consider the design space in which computational assistance augments and enriches people's intellectual work~\cite{Heer1844}. Opposed to our framework, these guidelines do not consider incorporating interactive facets into the model itself to enable efficient interaction.
%There also exist a vast literature on the efficient elicitation of user feedback for predictions of machine learning models~\cite{stumpf2009interacting} and the UX for machine learning~\cite{fails2003interactive, amershi2014power,yang2018machine}. While most related work concentrates on iterative model improvements, many findings can be formulated in the context of the interactive collaboration framework. 
%We further note similarities to the concept of explanatory debugging by Kulesza et al. that relies on interactions with a model~\cite{kulesza2010explanatory}, and which they find can lead to better personalization and improved mental models~\cite{kulesza2015principles}.

%Another important aspect of our work is that the interpretable parts of a model can act as explanations for rules of behavior that models learn. This kind of explanation has been shown to improve model personalization~\cite{bostandjiev2012tasteweights} and explainability~\cite{caruana2015intelligible}, while failing to provide explanations can inhibit development of mental models in users~\cite{lim2009and}. It is also known that explanations should not overwhelm a user and many previous approaches thus select less complex models~\cite{lacave2002review} or aim to reduce the feature space of a trained model~\cite{craven1997using, yang1997comparative}. Opposed to this, our proposed framework is agnostic to the model complexity, since the explanations are built into the model.

%Sacha et al. point out that only few works consider the model development as part of the visual analytics pipeline~\cite{sacha2019vis4ml}. In fact, the visualization of intermediate result has been pointed out as one of the promising future direction for visualization for machine learning~\cite{endert2017state} and has mostly been used to interact with data during time-intensive analysis pipelines instead of as explicitly modeled part of the interaction~\cite{stolper2014progressive}. There has also been a distinct lack of visual tools designed for non-experts that are not used as teaching tools~\cite{hohman2018visual}.

%\subsection{The Visualization Techniques}

%The development of methods for interactive, but not collaborative, visual interfaces has been an active field of research, as summarized in recent review papers~\cite{endert2017state, liu2017towards, lu2017state, hohman2018visual}.
%The visual approaches to integrate an expert's domain knowledge range from user-guided instance and feature selection~\cite{}, interactive parameter configuration~\cite{}, to active~\cite{holzinger2016interactive,cohn1996active}, and augmented-based learning~\cite{oblinger2006augmentation}.

%The visualization techniques relevant to our goal aim to understand how blackbox models work, how they perform under varying conditions, and how to debug and improve them.
%A step towards better model understanding is Google's \textit{What-If} tool~\cite{whatif}. Such counterfactual explanations~\cite{wachter2017counterfactual} allow to investigate changes in the outcome of a model for different inputs, thereby increasing trust and interpretability.
%This is especially of interest when models get increasingly complex, as it appears for deep learning approaches. One frequent proposal is to visually explore model internals and behavior to better understand them, as has been done for recurrent networks under varying conditions~\cite{strobelt2018lstmvis}. 
%Other methods focus more on debugging errors~\cite{zhang2019manifold, strobelt2018debugging, krause2017workflow} and only visualizing the necessary parts to find and explain them, instead of giving in-depth insights into hidden states.

%While many interpretability approaches concern classification problems~\cite{krause2017workflow,tam2017analysis} and can be applied to multi-modal input and output types, recent proposals for text have not yet converged towards a single set of techniques. Especially text-based problems such as entailment~\cite{liu2019nlize}, question answering~\cite{kwon2019retainvis}, and translation~\cite{strobelt2018debugging} have been approached by different visualization strategies. Following their insights that high-dimensional vectors are not interpretable, our use-cases do not include any visualizations of the hidden states. Instead, we focus the visualization efforts on those aspects of a model that can be readily understood by non-expert users. 

%We further identify similarities between collaborative approaches and the concept of models as a team member. Here, studies have shown that interactive models can improve the accuracy of studies~\cite{jordan2015machine}, facilitate interactions between multiple team members~\cite{siangliulue2016ideahound}, and improve the models themselves~\cite{fogarty2008cueflik, caruana2006meta, cohn2003semi}. Some recent work even aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating}. Thus, designing the model as a team member rather than a static resource can vastly improve outcomes. 

% \subsection{The Visualization Techniques}
% % Debugging/Analysis
% In this section, we contextualize the methods we applied to develop our use-cases within the related work and present alternative analysis and visualization approaches. A more general overview on combining machine learning with visual interfaces can be found in recent review papers~\cite{endert2017state, liu2017towards, lu2017state, hohman2018visual}.

% Interpretation of machine learning models is of particular interest to the visual analytics community, since visual techniques allow to better explore the behavior of complex models~\cite{zhao2019iforest, strobelt2018lstmvis} and to debug errors~\cite{zhang2019manifold, strobelt2018debugging, krause2017workflow}.
% Visual analytics can be applied to increasingly multi-modal input- and output-types. While many interpretability approaches focus on classification problems~\cite{krause2017workflow,tam2017analysis}, recent visual analysis means for text have not yet converged towards a single set of techniques. Especially text-based problems such as entailment~\cite{liu2019nlize}, question answering~\cite{kwon2019retainvis}, and translation~\cite{strobelt2018debugging} have been approached by different visualization strategies. 
% Following insights\rk{which insights?} from these papers, our use-cases do not include any visualizations of the high-dimensional hidden states. Instead, we focus the visualization efforts on those aspects of a model that can be readily understood by non-expert users.

% % Means to end
%\rk{I dont understand this part}
% Other inspirations of our presented use-cases originate in research on interactivity between user and model in computational social science. Here, the explainability often comes from the results itself instead of the process, and improved models can improve the accuracy of studies~\cite{jordan2015machine}, facilitate interactions between multiple team members~\cite{siangliulue2016ideahound}, and improve the models themselves~\cite{fogarty2008cueflik, caruana2006meta, cohn2003semi}. Some recent work even aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating}. Thus, designing the model as a team member rather than a static resource can vastly improve outcomes. 

% % Active Learning
% We differentiate our approach from work on interactive systems that aim to train models from the ground up, for example using different active learning techniques~\cite{holzinger2016interactive,cohn1996active} or systems that can be used to efficiently develop rule-based models from the ground up~\cite{oblinger2006augmentation}. 

==> Latvaria(IEEEVAST2019) (2)/src/032-latvar.tex <==
\section{Rearchitecting models to enable collaborative semantic inference}
\label{sec:latvar}

Interactive collaboration requires interpretable model hooks that enable semantic collaboration. From the machine learning side, these hooks can be implemented as discrete latent variables. During the prediction, or \emph{inference}, process, the variables take on explicit and understandable values. To illustrate this process, consider a hook resembling a lever that directs a train towards a left or right track, as shown in Figure~\ref{fig:latvar}. A model is predicting where a train will end up. Without the hook, the model can predict the end position accurately, but it is not clear how it will get there (top-left). Similarly, once the train reaches the top of the tracks, the model cannot explain how it got there (bottom-left). With the hook, however, the prediction explicitly exposes the lever decision. That means that it is predictable to the user whether the train will take the left or right branch (top-right). Once the train is at the top of the intersection, the user can look at the position of the lever to find the path the train has taken (bottom-right).

%In previous work, we have studied debugging tools for sequence models in order to examine predictions and conduct what-if analyses~\cite{strobelt2019s}. We found that the model architecture is a limiting factor. While we could change any intermediate representations and study outputs, small changes would often lead to major consequences. Furthermore, current systems only allow for \emph{forward} what-if analysis, whereas \emph{backward} inference, i.e., ``what internal decision would have led to a different output,'' is impossible.
%We propose using model "hooks" to target these issues by exposing internal model decisions. 

\begin{figure}[t!]
    \centering
    \includegraphics{figs/latvaria_train}
    \caption{The advantage of latent variables is the transparent reasoning process. CSI requires model reasoning, illustrated by a lever that dictates which turn a train is taking. In the forward inference direction, we know in both cases where the train will end up, but only the lever allows us to know what path it will take. Similarly, in the backward inference direction, we know where the train originated, but only the lever shows the track it took to get there.}
    \label{fig:latvar}
\end{figure}

To formally describe hooks, we consider the problem of generating a sequence of words $y_1, \ldots, y_T$ that is conditioned on an input $x$ using a deep model. In the exemplary problem of document summarization, $x$ represents a long document and $y$ the summary. 
A forward-only deep sequence model defines a conditional distribution to predict one word at a time, $p(y_{t+1}\ |\ y_{1:t}, x)$ while considering all previously generated words. 
In the collaborative approach, the deep sequence model is extended to expose intermediate terms as latent variables $z$. In the summarization example, this could be the decision what words in an input are considered important enough to be included in a summary. 
The architect defines $p(y_{t+1}\ |\ y_{1:t}, x)= \sum_{z} p(y_{t+1}\ |\  y_{1:t}, x, z) \times p(z\ |\ y_{1:t}, x)$ for the latent variable $z$. That means that the model considers all possible values of $z$ to make a prediction. In the train-lever example, that means we can run the inference process to compute the best lever position by looking at which of the two positions would lead to a better final position as judged by the model. 

This decision splits the black-box into multiple parts: a \emph{prediction network}, $p(y_{t+1}\ |\  y_{1:t}, x, z)$, that predicts the next word, and a \emph{hook network}, $p(z\ |\ y_{1:t}, x)$, that predicts the value of the latent variables $z$. 
Because this model is probabilistic, we can also perform posterior or \emph{backward inference}. This gives $p(z\ |\ y_{1:T}, x)$, the distribution of $z$ after taking into account the entire output, i.e., the text summary. 

Another example of a collaborative interface could be for semantic image synthesis~\cite{chen2017photographic,wang2018high,Park2019semantic}. In this application, a user-defined input $x$ describes high-level features, for example, the location of grass and sky, and a neural network generates the corresponding image. In this case, $y$ is an image and not a sequence of words. The current approaches do not allow iterative refinement through interaction with an image and are limited to changing the input and generating a completely new output. A collaborative approach to the same problem is GANPaint~\cite{bau2018gandissect}, which uses a hook network to associate parts of the latent space of an image-generating model with the semantic features and exposes a modification interface to the user.

%For example, Hughes et al. develop a model for the classification of the correct antidepressant for a patient that constrains a set of latent variables to act as the explanation~\cite{hughes2018semi}. A visual interface for this model could enable the interaction with groups of these variables as an assistant to the doctor. 

In a real-world example of a hook-network, Google Translate recently introduced a semi-collaborative approach to prevent gender-discrimination in translation systems. By treating the gender as a hook, they can present both possible options whenever the gender in a language is ambiguous, for example in Turkish. This approach allows a user to pick the translation they want.

The model hooks represent ways in which users can constrain and direct interpretable predictions in otherwise end-to-end black boxes. They are extensions of otherwise well-performing models to expose the latent variable, co-designed by experts in interaction design, visualization, and machine learning. 
They have to decide on the model hooks, desired interactions, and the associated visual encodings. While some guidelines have been developed for interaction design for machine learning~\cite{fails2003interactive,stumpf2009interacting,amershi2014power,yang2018machine}, they focus on designing machine learning methods where the model performs complementary tasks to the user, or where the user interacts with black-box models. In contrast, CSI enables the study of interaction design for models that approach the same task as the user. 
One important question that requires further study is how many hooks are actually useful to a user. As more latent variables are designed and incorporated into a model, the training process becomes increasingly more challenging and the model performance might degrade. Moreover, the increase in potential user interactions with additional hooks might overwhelm users. As a consequence, we focus on a model with a single hook throughout our use case and show how a single hook can already enable many powerful interactions. 

We now describe our co-design approach for a CSI system for document summarization and present the lessons we learned from our CSI co-design process in Section~\ref{sec:process}.



==> Latvaria(IEEEVAST2019) (2)/src/04-captioning.tex <==
\section{Use Case 1: A Collaborative Captioning Model}
\label{sec:uc1}

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth, draft]{"figs/LSTM_S2S_Latvaria_Levers"}
    \caption{\sg{Screenshot todo} Interface overview for captioning. }
    \label{fig:cap-overview}
\end{figure}

We choose image captioning as the first collaborative interface. Image captioning describes the problem of generating a description of an image that accurately captures its content. From the machine learning side, this problem is typically addressed with a sequence-to-sequence model with attention, which represents which part of an image the currently generated word focused on~\cite{DBLP:conf/icml/XuBKCCSZB15}.
Imagine a user Anne, who wants to use an interface, powered by a captioning model, to help her generate captions. With an unmodified forward model, we can design an interface where Anne can upload an image and the model suggests a caption. However, if Anne does not like the caption, she needs to post-edit the suggestion to her liking. Moreover, if the model focuses on the wrong object in the image, Anne has to write the entire caption from scratch. There is also no visual indication if a caption captures all the information available in the image. 

%use-case ideas: user wants to create captions, loads image, runs model, reads result, not satisfactory, adds and rearranges detected objects in the image, reruns model, better output, one wrong part, user makes corrections (also corrects attention), models shows most suitable input to achieve that, user again edits input, runs model, is satisfied with output.

We can address some of these issues without a modified model. Following insights from mixed-initiative writing assistants~\cite{babaian2002writer}, the interface should enable Anne to request model-input. For example, she should be able to write one sentence and have the model generate the second. Since this does not require any feedback towards the model, we can use a a constrained prediction similar to that in Seq2Seq-Vis~\cite{strobelt2019s}.

However, this interface does not prevent the model from focusing on objects that Anne might not want. For this, we need to be able to constrain the latent variable. A natural approach for the semantic interaction is to allow Anne to select objects in the input which tells the model what to generate. 
For this use case, we redefine the attention as a latent variable, similar to the approach by Deng et al.~\cite{deng2018latent}. This enables the forward semantic interaction through object selection. 

In the backwards interaction, Anne may want to know what part of the image she hasn't described yet. Since we have defined the attention over objects in the image, we can aggregate the attention over the entire collaboratively written caption\footnote{While the standard attention can be easily explained and visualized, the weights without a hook network do not directly correspond to explanations and are often ambiguous~\cite{lee2017interactive, Jain2019attention}.}. 


\subsection{Visual Design}


Notes:
- visual design considerations: 

- visual interface shows input-model-output. user can explore how input objects is connected to output objects.

- reduce visual clutter with edge bundling through proxies, emphasize objects in focus through highlighting/color coding.

- keep overview by hierarchical aggregation of input and output objects. words to sentences. (maybe more important for second use case)

- user can emphasize (but not enforce) objects/regions of interest in the input image, and output caption. - model takes this into account - collaboration.

- further user actions: add/delete/edit object regions in the input, edit captioning in the output - visual interface shows most suitable matches to achieve this output in the input space.


==> Latvaria(IEEEVAST2019) (2)/src/05-summary.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=\textwidth]{figs/ui_overview.pdf}
    \caption{Overview of the CSI:Summarization visual interface. (a) shows the input and overlays the currently selected content selection (blue) and the current content of the summary (red). (b) shows a connection between the input and the current summary through the attention, which shows explicitly where words in the summary came from. (c) shows the current summary, (d) shows proxy elements for both input and output groups. This enables an overview of a document, even when the text does not fit on one page. (e) allows the user to request suggestions from the model, (f) enters the edit mode and adds a new sentence to the summary. (g) toggles whether the text should be aggregated into sentences. (h) provides quick selections for the content selection (blue) by being able to match the red highlights, or (de-)select everything.}
    \label{fig:sum-overview}
\end{figure*}

\section{Use Case: A Collaborative Summarization Model}
\label{sec:uc2}



% Structure
% \begin{itemize}
%  \item summarization problem (High level)
%     \item Current use of interfaces with post-editing -- forward path
%     \item introduce hook 
%     \item describe interactions enabled by it for forward and backward as main features in the interface
%     \item Introduce additional interface features
%     \item maybe: introduce some design challenges
% \end{itemize}

% Summarization Problem (high level)
%We design a CSI approach for the problem of document summarization. 
We demonstrate an application of the CSI framework to the use case of text summarization. 
Text summarization systems aim to generate summaries in natural language that concisely represent information in a longer text. 
This problem has been targeted by the deep learning community using an approach known as sequence-to-sequence models with attention~\cite{DBLP:conf/icml/XuBKCCSZB15}. These models have three main architectural components: (1) an encoder that reads the input and represents each input word as a vector, (2) a decoder that takes into consideration all previously generated words and aims to predict the next one, and (3) an attention mechanism that represents an alignment between the current decoding step and the inputs. In summarization, the attention can be loosely interpreted as the current focus of the generation and can be visualized for each generated word~\cite{strobelt2019s}.\looseness=-2

% Current use of interfaces / post editing
Imagine an end-user called Anna, who wants to use an interface powered by a summarization model. Current deep learning models act in a forward-only manner, as described above; therefore the design space is limited to an interactive observation interface. This interface allows Anna to paste an input text and have the model infer an output summary. If Anna does not like the output summary, she can edit the suggestion to her liking, but it is not possible to reuse the model to check her changes. Moreover, if the model produced a bad or wrong output, Anna would have to write the entire summary from scratch. 

%Neural-network generated summaries achieve high levels of fluency and coherence, but can create factual mistakes or select unimportant content to summarize. That means that generated summaries require heavy post-editing from Users, which is currently designed in a disconnected process. 

% Hook
Applying the CSI framework by extending a well-performing summarization model with the previously defined hooks can address these issues. By tying the user's interactions to understandable reactions within the model, we can achieve three previously not possible interactions. The collaborative interface (1) \textbf{guides the model} towards important content, (2) \textbf{enables the dialogue} between human-generated and machine-generated output, and (3) allows a user to \textbf{review the decisions} the model would have made to generate a specific output, i.e.,\ what parts of an input text the model chose to summarize.

These changes require designing a semantic model hook that can describe the content that a model considers for a summary. %take into account in the forward step. Then, the backward step can explain what content has been taken into account by predicting the position of the hook. 
We base the hook on a similar model we introduced in our previous work on document summarization~\cite{gehrmann2018bottom}. Commonly applied neural summarization models have the ability to either copy a word from the source document or generate a word. In contrast to users who write a summary, this approach does not have a planning phase where the model decides what content should be able to be copied from a more global perspective. 
We, therefore, introduce a hook for each word in a document that expresses whether the model should be able to copy the word. By exposing the hook within the interface, we can describe the semantic interaction as the user-decision what content of a document is relevant for its summary. A detailed description of the forward and backward models can be found in Appendix~\ref{app:sum}.\looseness=-1

%Internally, the user-input constrains the prior probability of the hook network, which means that the model is implicitly guided towards the selected content.

%However, the model is not overly constrained and can still generate a summary in any order or phrasing. 

%During the backward step, the model can use an entire document and its summary to predict what words and phrases in the input have been covered. This coverage takes into account even words that have been paraphrased in the output. %\hp{this paragraph is dense and a bit boring - loosing attention of the reader} 

% \sg{Hen: describe interactions enabled by it for forward and backward as main features in the interface}
%We co-designed the model modifications and the visual interface \textit{CSI:Summarization} (Fig.~\ref{fig:sum-overview}) to showcase a prototype for a collaborative semantic inference system \hp{repetitive - edit}. We note that this system incorporates almost all the necessary interactions \hp{necessary for what? not clear} to illustrate the complexity and depth of the design space \hp{how can we be sure that we explored the whole design space? seems implausible} and we will discuss potential simplifications later (Sec.~\ref{sec:vih_design}). \hp{simplify or delete previous paragraph}

We now describe how Anna generates a summary by using our CSI interface to collaborate semantically with the model.

\begin{figure*}
    \centering
    \includegraphics{figs/latvaria_anna_01_v2.pdf}
    \caption{After selecting the content shown on the left, Anna requests the model to generate a fourth sentence (a). She does not like the suggestion and deletes it (b). To influence the model to generate about other topics in the input, she deselects the sentences that caused the suggestion (c). }
    \label{fig:uc_anna_01}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics{figs/latvaria_anna_02_rev.pdf}
    \caption{Anna wants to generate a sentence about the water on Mars and starts typing \emph{``The water is ...''} (a). This initiates the model to finish the sentence for her (b). To correct a minor mistake in the generated sentence, Anna activates the edit mode (c) and replaces the wrong word (d).}
    \label{fig:uc_anna_02}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics{figs/latvaria_anna_03.pdf}
    \caption{Anna selects a sentence that is currently not covered by the summary, indicated by the lack of a red border on the right (a). She generates a new sentence (b) and corrects the repeated phrase ``nasa scientists say'' (c). With the finished draft of her summary, she can now evaluate the coverage of the input document (d) and the final summary (e).}
    \label{fig:uc_anna_03}
\end{figure*}

\subsection{Collaborative Summarization: Anna's Story}

Anna intends to collaboratively write a summary of an article describing how scientists found water on Mars\footnote{The article can be found at \url{https://www.cnn.com/2015/03/06/us/mars-ocean-water-study}}. She begins by reading the article to assess what information is relevant and should be part of the summary. Then to begin the interaction, she selects the entire input text, shown by the blue highlights in Fig.~\ref{fig:sum-overview}a, letting the model know it is free to summarize any relevant part of the document. 

She starts the collaborative writing process by requesting that the model suggest three initial sentences (Fig.~\ref{fig:sum-overview}c). This triggers a forward inference of the model and a visual update that presents the suggestions to Anna. At the same time, the system computes a backward inference to show which part of the input has been summarized. Visually, the input text may be longer than the browser window, so we introduce a proxy element for each sentence in input and output (Fig.~\ref{fig:sum-overview}d). The covered words in the input are presented with a red underline and the proxies of the sentences with at least one covered word have a red border (Fig.~\ref{fig:sum-overview}a,b). The interface also visualizes the model ``attention,'' which shows which covered words were selected by the model at what step during the generation. The attention is visualized using grey ribbons that are aggregated across each sentence and connect the proxy elements. By hovering over one of the sentences or proxies, the interface highlights the relevant connections in yellow (Fig.~\ref{fig:sum-overview}b). 

Through these visual interactions with the output summary, Anna observes that the second input sentence (\emph{``scientists at nasa are one step closer to understanding how much water could have existed on primeval mars. these new findings also indicate how primitive water reservoirs there could have evolved over billions of years, indicating that early oceans on the red planet might have held more water than earth's arctic ocean, nasa scientists reveal [...]''}) splits into two different summary sentences (\emph{``primitive water reservoirs there could have evolved over billions of years, scientists say.''} and \emph{``early oceans on the red planet might have held more water than earth's arctic ocean.''}). It is common for summarization models to compress, merge, and split input sentences, but the user would not be aware of where the inputs for each summary sentence originate. By exposing the internal model decisions in a CSI interface, a user can immediately discover how the input connects to the output.\looseness=-1

From this suggested summary, Anna determines that the input focus of the system was correct, but that output text should elaborate on these sentences in more detail. She communicates this by first constraining the model to the 
currently focused region. She can match the content selection (blue highlights) with the result of the backward inference (red underlines) by clicking ``match'' in Fig.~\ref{fig:sum-overview}h.
 %This content is found during the backward step that the interface automatically triggered after presenting the suggestion. 
%She semantically interacts with the input mask and restricts it to all the sentences identified in the backward step for the current summary. 
With these constraints, she triggers the generation of an additional output sentence (\emph{``nasa scientists say that much of this water loss happened over billions of years, along with a loss of atmosphere.''}) (Fig.~\ref{fig:uc_anna_01}a). This suggestion is the result of a forward inference with her additional constraint on the model hook.\looseness=-1

Unfortunately, Anna is dissatisfied with the new sentence, so she removes it from the summary (Fig.~\ref{fig:uc_anna_01}b). To prevent the model from suggesting the same sentence again, she consults the backward inference and deselects the input sentence that had the highest influence on its generation by clicking on its proxy element (Fig.~\ref{fig:uc_anna_01}c). 
With this updated constraint, Anna generates another sentence (\emph{``water trapped in mars' polar ice caps has a much higher level of hdo than fluid water on earth.''}) that better captures her goals. (Fig.~\ref{fig:uc_anna_02}a). 

%Influencing the reasoning process of the model in this way is only possible by the semantic interaction with the hook that is enabled by the CSI model. 

Anna would next like to include more details to the summary, particularly about water found on Mars. The system allows her  to intervene in the output text directly. She starts writing ``the water is'' and then adds an ellipse (...) that triggers sentence completion by the model (Fig.~\ref{fig:uc_anna_02}b,c). The resulting sentence (\emph{``the water is very likely wet for a longer period of time than was previously thought, the scientists say.''}) is acceptable to her, but she now spots an error with the verb (\emph{``is''}) which should be in the past tense. She quickly corrects this output (Fig.~\ref{fig:uc_anna_02}d,e), which invokes a backward inference to the input document. By updating the red highlights in the input, the interface provides her with information about what content was selected was used to create this improved sentence. These interactions help her create a mental picture of the model behavior. 

Anna would finally like the model to help her generate a sentence about a region of the input that is currently not included in the summary. She selects a previously unused sentence in the input (\emph{``this ocean had a maximum depth of around 5,000 feet or around one mile deep, said villanueva.''}) (Fig.~\ref{fig:uc_anna_03}a), requests another forward inference, and approves of the resulting suggestion (\emph{``this ocean had a maximum depth of around 5,000 feet or around one mile deep, nasa scientists say.''}). However, she dislikes the repetition of ``scientist say'' (Fig.~\ref{fig:uc_anna_03}b). After entering the edit mode on the output side, she removes one of the repeated phrases (Fig.~\ref{fig:uc_anna_03}c). Upon leaving the edit mode, the interface automatically triggers another backward inference that updates which parts of the inputs are covered. Anna uses this information to evaluate how much of the document is covered by her summary. By looking at the computed coverage (Fig.~\ref{fig:uc_anna_03}d), she can observe which sentences are covered and analyze how many of the proxies have a red border. Her six sentences (Fig.~\ref{fig:uc_anna_03}e) summarize the original text pretty well. 

%We next describe Anna's actions in scope of the CSI actions between the model and the UI. 

%\subsection{Anna's CSI interactions}
%At first, Anna has to decide on a scope for the initial summary. 
%The forward step of the model generates three sentences that are presented to Anna (Fig.~\ref{fig:sum-overview}). 
%She can then click the \textit{add sentence} button. The second forward step then conditions the output on the constrained mask and generates a single sentence. The resulting sentence starts promising but yields some problems, so Anna decides to help out.

% \begin{itemize}
%     \item 1.1 - “request” tab: show attention for 1st sentence 
%     \item 1.3. - “latent” tab: show 2nd sentence
% \end{itemize}

% Although this problem has a different input type and use-case, we can apply most of the same design approach as the previous use case. A user Anne wants to use the collaborative interface to generate summaries. 

%She uses the \textit{edit} button on the incorrect summarization sentence and starts changing the parts that do not fit. 
%The annotations demonstrate which parts of the input are covered by her summary text. 
%Instead of editing suggestions, Anna can go one step further and add a new sentence entirely by herself. Similarly to the edit action, finishing the new sentence triggers a backward step, which shows that the sentence covered the sentence that Anna aimed to summarize. \sg{this does not match story, do we have another picture here?}

%As a third collaborative editing action, Anna can call on the model to finish a sentence. She remembers that there was something mentioned about the depth of oceans. She starts a new sentence with "the mars oceans had a depth of ..." and indicates by the final three dots that she wants the model to complete her sentence. Upon seeing the three dots, the interface triggers a forward step in the model that predicts words until end of the sentence. 
%\sg{picture}


% \begin{itemize}
%     \item 2.1. try with fwd model and selection mask (latent) only
%     \item Yields a funny result, user can post-edit
%     \item backward model updates its believe accordingly
%     \item 3.0 User can add a fully new sentence
%     \item 3.1 New sentence is not accounted for in the attention, but backward model updates correctly
% \end{itemize}



% Mixed initiative
%\hs{what is the follwing text? Redundant ?}


%However, this interface does not prevent the model from focusing on objects that Anne might not want. For this, we need to be able to constrain the latent variable. A natural approach for the semantic interaction is to allow Anne to select words in the input. In the summarization use case, the input can be hundreds of words long and the visual interface can assist Anne by allowing interactions with groups of words instead. Thus, the interface requires the aggregation of input and outputs. This has further implications on the visualization of the attention. \sg{...}




\subsection{Visual and Interaction Design}
\label{sec:vih_design}

We designed the text summarization prototype (\textit{CSI: Summarization}) such that text occupies the majority of screen estate as the central carrier of information for the task. Two central panels (Fig.~\ref{fig:sum-overview}a,c) represent input text and output text. Each text box represents words that are aggregated into sentences. Text highlights in the input show information about the model hooks and relations between input and output. %The blue highlights at the word and sentence level indicate the current selection that the next forward pass of the model should consider. The red underlines (Fig.~\ref{fig:sum-overview}a) and borders indicate what inputs the model considered if it had generated the current output text, i.e., the output of the backward pass. Yellow highlights while hovering show connections between an input and the corresponding output and vice versa. 
Neutral gray colors are used on the output side to clearly distinguish them from the blue colors that represent selections on the input (Fig.~\ref{fig:sum-overview}c).\looseness=-1

The input and output text are connected by a bi-partite graph that indicates model attention (Fig.~\ref{fig:sum-overview}b), which expands on previous work on visualizing and normalizing attention~\cite{strobelt2018debugging,linvisualizing}. %Similar to Seq2Seq-Vis~\cite{strobelt2019s}, the graph edges show what the model attended to during the forward inference. The attention is defined between all the words of input and output. 
Due to the length of source documents, displaying the entire graph is not feasible or informative. Therefore, we use two design elements to observe the full graph in a de-cluttered view: aggregations and proxies. First, we allow the aggregation of words into meaningful word groups, e.g., sentences, that can be dissolved on demand (Fig.~\ref{fig:iteration}d) if this level of detail is required. Aggregating words implicitly requires the aggregation of the attention which simplifies the graph. Secondly, we represent sentences by a vertical arrangement of boxes that are space-filling in height and which act as proxies for the full sentences. In that way, all sentences are always visible by their proxy, even when they are outside the display area. These proxies mirror selections and highlights of their related text boxes.\looseness=-1

\textit{CSI: Summarization} offers a range of user interactions. As a general principle, buttons trigger forward (left to right) actions (Fig.~\ref{fig:sum-overview}e) because a forward inference can change the output summary itself. Unintended changes to the output could confuse the user. To let users explicitly request updates instead of automatically intervening is inspired by similar mixed-initiative writing assistants~\cite{babaian2002writer}, where researchers found that this type of interaction is seen as least intrusive. %Moreover, the forward mode will change the summary, and unintended changes to the summary could confuse a user. 
All backward inferences are automatically triggered after exiting the edit mode by hitting enter. Since backward interactions do not change the content of the summary, the automatic invocation does not lead to accidentally overwriting important information. Users can define which sentences or words to consider for generating the next sentences by selecting them (blue color). Clicking on the bar on the right of an aggregation group selects or deselects the entire group. The same action is triggered by clicking on the proxy element of the corresponding sentence  (Fig.~\ref{fig:sum-overview}d). 

\begin{figure}[t!]
    \centering
    \includegraphics{figs/latvaria_iters.pdf}
    \caption{Visual design iterations for \textit{CSI:Summary}. (a) shows radio buttons for selecting a specific selection (content selection vs. backward model). In (b), we introduced a mixed mode that showed the user content selection in the final blue color and the result from the backward model with a red highlight (c). Underlines later replaced the dominant highlight. (d) shows an example of the complexity of the attention graph without any aggregation.}
    \label{fig:iteration}
\end{figure}

The interface additionally provides three selection templates  (Fig.~\ref{fig:sum-overview}h) for convenience: select all sentences, select no sentence, or select only those sentences that match the selection from the backward step (match red and blue). For the forward pass, the selection can be used to either initialize a new summary with a user-selected number of sentences (\texttt{init with}) or to add a sentence to the existing summary (\texttt{add sentence}) (Fig.~\ref{fig:sum-overview}e). On the output side, sentences can be deleted or edited by clicking the \texttt{edit} and \texttt{delete} buttons at the end of each sentence. %After finishing an edit on the output side, the backward model computes the corresponding input text that is being referred to, and the interface underlines the input accordingly. Similar to editing, the user can also create new sentences  (Fig.~\ref{fig:sum-overview}f). A new sentence can be completed by the model by typing an ellipse (...) end exiting edit mode. 

% We also considered an alternative interface in which a user can directly edit and add text without entering a separate mode. However, our decision to have a separate mode has three major advantages. Upon exiting the edit mode, we can provide (1) problem-specific automatic text formatting, and (2) look for the text finishing request \emph{...}. (3) The exiting of the edit mode is an explicit signal to initialize the backward step, which otherwise would need to be a separate button. 

\subsection{Design Iterations}


During the creation of the prototype, we explored multiple designs for model hooks, visualizations, interactions, and their integration. Overall, we found that CSI systems are more difficult to design because of the, sometimes competing, interactions between all these elements. We want to highlight one example for each of the elements. 

On the model side, our initial backward inference had good accuracy but did not reveal useful information within the interface. Only after re-allocating efforts to train a different model with a much higher performance did the backward model match the human intuition. Since model hooks complicate the design of the machine learning models, it also complicates their training process. Issues, such as the one described above, are only uncovered with the visual interface. 

On the visualization side, we explored multiple different designs for the input selections presented in the interface. The selections we currently show are (1) the selection that was used for the most recent forward step, (2) the selection that was returned from the most recent backward step, and (3) the sentences that the user is selecting for the next forward pass. In our first iteration, we aimed to show all of them in separate views (Fig.~\ref{fig:iteration}a), and additionally have a view that highlights their intersection (Fig.~\ref{fig:iteration}b,c). Internal tests revealed that only the combined view was useful to users to avoid having to switch forth and back. We, therefore, replaced the different views by the current more natural and coherent use of red and blue highlights within the same view. In conclusion, this design iteration provides a good example of the prevalent visualization challenge how to encode necessary information for the targeted user group. For CSI interfaces, the task is severe because of the major difference in abstraction between model internals and end-users intuitive understanding.

On the interaction side, we found that requesting the model to generate words without a constraint on the minimum or the maximum number of sentences often led to output that was unreasonable to users. The model architects on our team pointed out that the training data for summarization models rarely contains examples where the summary is longer than three sentences. Forcing a model to generate longer summaries than it was trained to generate led to the degradation in output quality. We also found that users had more control over the content of a summary if they iteratively built up a summary from a short initial suggestion instead of suggesting a lengthy summary and letting the user change it afterward. Our current modes combine these findings by designing the interaction after discussions with our model architects and visualization experts. 
The first interaction initially generates a small maximum number of sentences. This both leads to better model output but also lets users explore the output space more effectively. Similarly, adding one new sentence at a time by incorporating previous sentences as prefix context and allowing users to select the content enables users to quickly generate and review new content.

%\hp{can you add some text and a figure with design iterations for visualizations and interactions? currently, they seem to focus exclusively on the model}


% \sg{Hen: Introduce additional interface features}

% \sg{Hen: maybe: introduce some design challenges}


% \sg{Hen, visual design similarities, attention}

% Notes:
% - visual design considerations: 

% - visual interface shows input-model-output. user can explore how input objects is connected to output objects.

% - reduce visual clutter with edge bundling through proxies, emphasize objects in focus through highlighting/color coding.

% - keep overview by hierarchical aggregation of input and output objects. words to sentences. (maybe more important for second use case)

% - user can emphasize (but not enforce) objects/regions of interest in the input image, and output caption. - model takes this into account - collaboration.

% - further user actions: add/delete/edit object regions in the input, edit captioning in the output - visual interface shows most suitable matches to achieve this output in the input space.

% \subsection{Co-Design Iterations}

% \begin{itemize}
%     \item Aggregation for more efficient semantic interaction
%     \item Visual Codesign: backward model did not make sense, needed to update it. Vis helped identify when it was ``good enough''
%     \item Multiple modes -> one mode
%     \item Visual Metaphor: Blue/grey for selecting output vs input needed to be separated 
% \end{itemize}

==> Latvaria(IEEEVAST2019) (2)/src/06-process.tex <==


\section{Towards a Co-Design Process for CSI Systems}
\label{sec:process}

% \begin{figure}
%     \centering
%     \includegraphics{figs/latvaria_process.pdf}
%     \caption{The CSI process model. The steps describe the core development process \hp{what does that mean? explain} and explicitly encode the co-design between machine learning and visualization experts.}
%     \label{fig:process}
% \end{figure}

During the implementation of the \textit{CSI:Summarization} prototype we developed an understanding of how an integrated design process for CSI systems could look like and also experienced its limitations. We discuss our insights as learned lessons.

\paragraph{Prioritize collaborative output.}
CSI systems enable joint production by model and end-user together. The resulting output should be the central element for developing visualization and interaction ideas. It is essential to evaluate if a \textit{CSI approach is beneficial} for the given task, e.g., a face recognition model used to unlock a cell phone does not benefit from the CSI approach as no shared output is produced. Since \textit{CSI methods are decision-shaping}, they require human oversight and interventions and are thus not suited for processing massive data. Moreover, since CSI interfaces are targeted at end-users, the visualization can be domain-specific but should abstract model-internals in an intuitive way. Finally, \textit{no side should dominate over the other} to allow model-human collaboration, which should be reflected in the visualization and interaction design -- e.g., allowing equal easy access to triggers for human input and model suggestions. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/latvaria_process_v2.pdf}
    \caption{CSI interfaces require a design process that spans machine learning and visual interaction design. The feedback loop is used to produce interpretable semantic representations that inform the 
    reasoning procedure of the model while providing useful visual interaction. }
    \label{fig:loop}
\end{figure}

\paragraph{Co-design requires continuous evaluation.}
 In the development of the summarization system, there was a \textit{constant negotiation between visualization requirements and model capabilities}. This process led to iteration on the question: ``does this visual encoding help the end-user collaborating with the model?'' and ``which additional model behavior do we need to help to encode relevant information?''. Fig.~\ref{fig:loop} illustrates how this continuous co-design play forms a bilateral relationship between model design and visualization design. CSI systems, like most visual analytics systems, can help to \textit{reveal model problems} immediately. If, for example, a specific model hook is performing so poorly that it cannot facilitate the user's mental model, it will be immediately revealed. On the other hand, requirements for a \textit{visualization might over-constrain a model} such, that it breaks. E.g., creating a system for poem writing which should suggest lines of text that rhyme, even for human entered text, might over-constrain the model. CSI systems are about to find the middle ground between what would be ideal for a user interface vs. what would be possible with the underlying ML model.
 
 
\paragraph{CSI may be a worthwhile investment.}
Since CSI is centered around a single abstraction that should reflect the mental model that an end-user has of a problem, we pose that \emph{machine learning needs to learn about interactions}. There is currently a limited understanding of the space of easily trainable hooks and interaction strategies. Since machine learning techniques do not natively consider bidirectional interactions with end-users, the visualization, interaction design, and machine learning experts need to teach each other about desired interactions and the limits of deep models. Deep learning models with hooks thus lead to an increased development complexity for both machine learning and visualization experts. However, during the development of the summarization use case, we also experienced that \emph{CSI has a learning curve}. While CSI systems are individualized to a problem and thus one-of-a-kind systems, most of the techniques are transferable and the team can apply the insights gained from one CSI project to the next one. 
Moreover, the long-term benefits of the increased control over models can justify the additional development complexity, especially considering that many applications in industry are used for many years. As shown in our summarization example, the CSI methods can even lead to more structure and subsequent improvements in outcomes. 


% submission lesson 3:
% \paragraph{Machine learning needs to learn about interactions.}
% An essential part of creating visual CSI systems is to \textit{use high performing models}. Because the models are now part of the visualization and interaction design, the usability of a system highly depends on the model performance. The reason why CSI systems are not common is that deep learning models only recently surpassed the performance levels necessary for effective collaborative approaches. Moreover, \textit{machine learning techniques do not natively consider bidirectional interactions} with users. It is thus on the visualization and interaction design experts to teach model architects about desired interactions, and the model architects need to teach visualization experts about the limits of the models.\looseness=-1 


% Super old: 


%Without these high-performing models, the users do not benefit from the dialogue.  
% As a consequence, we needed to extend state-of-the-art summarization methods as part of the development of CSI:Summarization to make it useful. 

%The same is true for the data. We recommend to \textit{use appropriate small data} for fast iterations and to allow proof-of-concept implementations. This data might be synthetic if it can help to test the visual encoding in combination with the model. Finally, it is similarly crucial to \textit{think about appropriate large data} that allows creating a real-world CSI system. E.g., it will not satisfy a user to use a large general English language model trained on financial news if the application is a co-writing tool for children's books.
%\rk{maybe find better ending for this section.}

% Consequently, most of the key features in CSI visual interfaces (Fig.~\ref{fig:intmodel}c) require a counterpart within the model. We therefore see the visualization and interaction design as the first step in systematically creating CSI systems involving both model architects and visualization experts. 




%\hs{-- old -- }

% The co-design of machine learning and visual interaction requires a structured process. Unlike passive or interactive observation interfaces (Figure~\ref{}(a) and (b) \hp{ref to Fig. 2}), the majority of features in interactive collaboration interfaces (Figure~\ref{}(c) \hp{ref to Fig. 2}) require a counterpart within the model. It is thus challenging to avoid over-engineering either the visualizations, interactions, or model features.  In this section, we describe a process that we acquired over the course of this and previous projects \hp{add ref}, including lessons learned for each step. Our design process extends the visualization design process described by Sedlmair et al.~\cite{sedlmair2012design} to explicitly encode the roles of the machine learning and visualization experts. An overview of our process is shown in Figure~\ref{fig:process}.
% While our CSI design process describes the \emph{actions} taken to develop collaborative interfaces, the nested blocks and guidelines model~\cite{meyer2015nested} can be applied to the reflection process, where the two roles are reflected in the algorithm and technique blocks. \hp{you need to describe this in more detail, do not assume the reader knows that reference}

% \paragraph{Interaction Design}

% The first principle of mixed-initiative interfaces (MII) \hp{why do you use this term? I thought we are describing the CSI process? avoid adding more jargon} is that the interaction with a model should add value~\cite{horvitz1999principles}. That means that we need to carefully evaluate the potential interactions without an interface \hp{everything has an interface, not sure what you mean}, but also the potential interactions without backwards interaction \hp{sentence is unclear}. If this constrained design space comprises the desired interactions for a use-case, a non-CSI system may be sufficient. \hp{this paragraph makes no sense to me} 

% Unlike previous examples of intelligent writing assistants, the model and user are not solving complementary, but different problems~\cite{babaian2002writer} \hp{what? and how does this fit with our process?}. Instead, both agents, user and model, can actively work on the refinement of a shared solution (Step 9 in MII) and the user can constrain and influence the intermediate reasoning of the model \hp{you are off in philosophy land - none of this makes sense to me}. To design the semantic interaction, we recommend staying close to the mental model the user has of the problem. In the case of summarization, writers tend to select relevant content first and rephrase it in a second step~\cite{anderson1988teaching}. By constraining the model to follow the same reasoning process, we can develop a more intuitive interface. \hp{you need to describe the process in general terms. only use summarization as an example.}

% Upon agreement on the semantic interaction, both parties need to develop a protocol to be used in the interface between model and visualization  \hp{what do you mean?}. Often, machine learning and visualization experts use different language to refer to the same concepts and this can lead to misunderstanding in the API development \hp{this is a secondary issue that should have nothing to do with the process}. Similar to test-driven development, it is thus helpful to identify simulated payloads \hp{what?} the model will return for specific requests from the interface. Then, both sides can program against this blueprint. 

% \hp{this whole section needs to be rewritten. right now, this makes no sense, and it does not describe or justify the process.}

% \paragraph{Visualization Design}

% \hp{I don't like the term 'implementation' in the process model. use 'visualization design' and 'model design' instead}

% Identifying the user's language and mental model plays a significant role in identifying the scope and method of visually presented information.
% We found it useful to follow the design study strategies to develop and implement the visual encoding. \sg{which guidelines?}
% Using the wrong visual language can lead to a mismatch with the user's mental model or cognitive overload. \hp{what do you mean by visual language? visual encodings?}
% E.g., it is not necessary to present a neural network architecture diagram if the focus is on understanding which linguistic features a model captures.

% Especially for CSI systems, a constant negotiation about what the visualization \hp{avoid the term UI when you talk about visualizations} would require and what the model can deliver is at the core of visual design. Sometimes, the model quality might prevent some features \hp{why? explain}, sometimes the model output (even of a hook) might be complex and require another visual abstraction \\hp{another, or a different one? I am not sure what you mean}. We need to consider how a model can add meaningful content, and modify existing content without ignoring the user's input. \hp{???}

% The focus of CSI systems is to create a joint output created by model and human. The output should be the central element of developing interaction ideas. To allow true collaboration, no side should dominate over the other, which should be reflected in the visualization or interaction design -- e.g. allowing equal easy access to triggers for human input and model suggestions. 
% During the design of the interaction, the system should keep a working memory of the recent interactions (step 11 in MII \hp{what are your referring to? do not assume the reader knows the references}) to visualize changes over time. \hp{this is the section about the visualization design, not interaction design. stay focused on one or the other}

% % \begin{itemize}
% %     \item \sg{Hen?}
% %     \item During the design of the interaction, the system needs to keep a working memory of the recent interactions (step 11 in MII) to visualize changes over time. 
% %     \item We need to consider how a model can (1) add meaningful content, and (2) modify existing content without ignoring the User's input. 
% % \end{itemize}

% \paragraph{Model Design}

% The first task of the machine learning expert is to implement the forward model for the specified task. Often, we found it more effective to use simulated data and an easier model to rapidly develop the interface. For example, in LSTMVis \hp{add ref}, we used a simple language of opening and closing parenthesis and in Seq2Seq-Vis \hp{add ref} the problem of formatting dates. \hp{how did this help?} 

% Another advantage of starting with the forward model is the faster iteration time. If the forward interactions do not lead to sensible output, it is likely the model's fault. We thus recommend defining clear measures what constitutes a successful model that correspond to whether the visual metaphors align with the mental model of the problem \hp{of the user. a problem has no mental model.}. In Seq2Seq-Vis, this helped us debug errors in how the attention was computed and returned to the visual tool. \hp{what did we do specifically? describe}

% Only once the forward model works as intend, we can develop the backwards interaction \hp{is this always true, or a recommendation?}. Latent variable models in deep learning are not a solved problem \hp{this sounds weak}. The machine learning expert might have to extend existing ideas to incorporate the desired interaction design \hp{weak}. For example, the bottom-up attention for summarization in our presented use case is originally restricted to forward interactions. We developed a second backward model specifically for the use case that can predict coverage of a document, given the summary. 

% \paragraph{Small-Scale Test}

% Collaborative interfaces are aimed at Users \hp{why? we did not state this until now, and I don't believe this true}. Neither machine learning nor visualization experts might be qualified to reason about a tool's usefulness \hp{definitely false! delete!}. Often, the first prototypes of an interface are far from usable to study the intended interactions. Therefore, after each implementation step, we inquire feedback from experts that help us reshape the design. \hp{this is generally true in iterative design. what's special about our process?}
% For LSTMVis, we collaborated with experts in genomics and linguistics who could verify whether the tool's findings matched their intuition. \hp{I would be careful, since for this paper we did not have external experts.}

% We suggest going through this process at least three to five times to refine the interactions, model, and interface \hp{why? seems arbitrary}. The findings from these design iterations correspond to the ``design iterations'' section in an application-focused design study paper. \hp{not very useful advice}

% The small-scale tests can further help to identify failures early. Since adding hooks to a model increase its complexity, the resulting model might perform well enough for a collaborative interface. That means that design iterations should not only occur on the visual side but also on the machine learning side. \hp{there is a separate section on the model design, do not mix them} In fact, our first backward model for summarization did not perform well enough for the interface. It became useful only after we improved its prediction accuracy on unseen data from 76\% to 93\%. \hp{maybe move this to model design section}
% %Moreover, our plan to develop a second use case for an image captioning problem failed after we ran into problems that would require extensive research to develop appropriate machine learning models. 

% \paragraph{Long-Term Study}

% \hp{I don't like this, since we are not doing it for this paper. Plus, this is all very generic advice that has nothing to do with CSI}

% Past work has identified that findings of focused studies of interpretability methods rarely generalize and scale poorly due to visual overload~\cite{poursabzi2018manipulating, lage2019evaluation}. Thus, A/B tests are insufficient to measure the impact that explanations have on users. Sometimes, interpretability methods even pick up on spurious correlations in inputs that lead to confounding results~\cite{SanityNIPS2018, 2017arXiv171100867K}. To address this problem, the effectiveness of different methods needs to be carefully evaluated in real-world or proxy tasks~\cite{doshi2018considerations}. 

% Since interactive collaboration is aimed at the User, we aim to gather feedback from the actual users of the tools by releasing the tools to the public. 
% We gather the following measures over time: (1) Do people use the tool as intended?, (2) Do people use the tool for unintended purposes? (3) Does the release inspire further research?
% Long-term studies do not replace focused gathering of results and the evaluation of the effects of the tool on users. They do, however, allow for the evaluation on a much larger scale both in time and sample size. 

% We found that this strategy works especially well for measure (2). While LSTMVis was focused on analyzing language models in natural language processing, we found that the open-source release sparked its use for time-series analysis for economic problems or sequence analysis in biology. By only conducting focused evaluations, we would not have been able to find these unintended use cases.  

% \hp{this section either needs a complete rewrite or we should nix it. Right now it is so general as to be useless.}
 
%  %Some recent work has tried to automated the iterative development and testing-process by including user-studies within the development cycles~\cite{lage2018human}.

==> Latvaria(IEEEVAST2019) (2)/src/07-discussion.tex <==
%\section{Discussion}
%\label{sec:disc}

% Advantage of our model




%A collaborative approach can further integrate the model as an active team member instead of a static entity. This interpretation can help to facilitate interactions between multiple team members~\cite{siangliulue2016ideahound}, and improve the models themselves~\cite{fogarty2008cueflik, caruana2006meta, cohn2003semi}. 
 %Here, designing the model as a team member rather than a static resource can vastly improve outcomes. 

%It is increasingly important to consider ethical implications of designing algorithmic interactions with humans~\cite{wilks2010close,williams2018toward}.
%The interpretability-first approach in collaborative interfaces can help to highlight fairness and bias issues underlying the data or a model~\cite{hughes2018semi, holstein2018improving}. By interacting with the visual interface, the users can avoid unethical output and similarly to prevent factual errors. Google translate recently introduced a semi-collaborative approach to prevent gender-discrimination in translation systems. By treating the gender as a hook, they can present both possible options whenever the gender in a language is ambiguous, for example in Turkish. This approach allows a user to pick the translation they meant, given the wider context and their intrinsic knowledge.

%\hp{I am not sure this is the kind of discussion that gets reveiwers excited.}


%Imagine that a recipe model learns the human bias that kale is inferior to spinach and always includes spinach instead of kale in recipes. An analogous argument can be made for the development of characters in story where a model could discriminate against minorities or gender. However, by explicitly modeling character (or vegetable) choices and presenting them to the user as interactive prediction, this discrimination can actively be prevented from happening.

% Finally, the strategy exploits the exponential search space of a model more efficiently. Models typically produce boring outputs that have a high probability but are not very interesting. Humans perform better at creative tasks and can guide the model towards more interesting outputs. 

% Many text-generation tasks do not offer one correct answer. Although tasks like text summarization and image captioning are often trained with a maximum likelihood objective that optimizes each input to produce one professionally written gold target, one input can have multiple valid outputs. Depending on user preferences, a generated text could use different tenses, describe an event with a different sentiment, or focus on completely different parts of the input. There is an additional issue in that models typically learn biases underlying the data. For example, if human-written summaries have a strong focus on the male actors of a story, the model is likely to learn this wrongful bias. There is ample research in de-biasing datasets and models, but this requires knowing of the existence of these biases. Google translate recently introduced the approach to present both possible options whenever the gender in a language is ambiguous, for example in Turkish. This approach allows a user to pick the translation they meant, given the context and their intrinsic knowledge. 

% Limitation

%However, collaborative interfaces come at a cost. Although this framework aims to explain some of the possible designs, we currently do not understand much about the design of the semi-global aspects that control output in an interpretable way. These aspects, which we refer to as interpretable hooks in the framework, also lead to an increased implementation complexity. 
%Moreover, collaborative interfaces, for example predictive keyboards, could introduce unwanted biases by guiding the user towards what the model has learned~\cite{arnold2018sentiment}. Furthermore, the use of these models is restricted by available human resources for the tasks they complete, whereas fully autonomous models require less supervision. In many use cases this is a benefit since it forces users of a model to double-check its outputs, but in others it might restrict the scalability. Finally, it is currently not well understood how these models can be formally evaluated without large-scale human studies. 

%\hs{discuss simpler summarization interface for End-User }

% Ethics

%It is increasingly important to consider ethical implications of designing algorithmic interactions with humans~\cite{wilks2010close,williams2018toward}. %We base our ethical argument on the framework by D\"orr and Hollnbuchner who discuss ethical challenges in algorithmic journalism~\cite{dorr2017ethical}. In their framework, each user aims to uphold the principles of objectiveness, transparency and accuracy, but is subject to external constraints that sometimes prevents moral action. An algorithm in semi-algorithmic content generation represents one such constraint, since it introduces an additional actor with their own moral guidelines. Typically, the algorithms are treated as relatively autonomous actors with delegated (moral) agency. As such, it is the responsibility of the creator and the user to ensure minimal contradicting behavior. 

% Autonomy

%TODO
%We further note similarities to the concept of explanatory debugging by Kulesza et al. that relies on interactions with a model~\cite{kulesza2010explanatory}, and which they find can lead to better personalization and improved mental models~\cite{kulesza2015principles}.

%We further identify similarities between collaborative approaches and the concept of models as a team member. Here, studies have shown that interactive models can improve the accuracy of studies~\cite{jordan2015machine}, facilitate interactions between multiple team members~\cite{siangliulue2016ideahound}, and improve the models themselves~\cite{fogarty2008cueflik, caruana2006meta, cohn2003semi}. Some recent work even aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating}. Thus, designing the model as a team member rather than a static resource can vastly improve outcomes. 

% Hughes et al. develop a model for the classification of the correct antidepressant for a patient that constrains a set of latent variables to act as the explanation~\cite{hughes2018semi}. A visual interface for this model could enable the interaction with groups of these variables as an assistant to the doctor. 

==> Latvaria(IEEEVAST2019) (2)/src/08-conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusion}

In this paper, we introduced a framework for collaborative semantic inference, which describes a design process for collaborative interactions between deep learning models and end-users. Interfaces designed within this framework tightly couple the visual interface with model reasoning. We applied CSI to develop a collaborative system for document summarization that demonstrates that CSI systems can achieve powerful interactions within an interface powered by a neural model.\looseness=-1 
%We finally drew on the lessons we learned in the development of this and other related work and developed a focused process model that describes the development of CSI interfaces. 

While previous studies have shown that explainability methods can mediate in an agency-efficiency trade-off~\cite{lai2018human,yin2019understanding}, none of them demonstrate a way for users to retain agency while gaining the efficiency benefits of models interaction. We believe this is due to the difficulty of engaging the user in the prediction process of a black-box model. We address this problem by designing semantic interactions as part of the model itself. While CSI does not solve problems with biased data and models or the lack of interpretability of models, it aims to expose important model decisions and facilitate collaboration between an end-user and the model to take these decisions. Further developments in interpretability research could be used in conjunction with CSI for a better overall model understanding.  

The CSI framework significantly expands the interaction design space over conventional interaction strategies for many deep learning models. CSI-style approaches have the potential for application especially in scientific or safety-critical applications where explainable AI may become mandatory. Moreover, since CSI treats the model as a team member, another area of particular interest are creative applications, where models can assist users in creating stories~\cite{fan2018hierarchical}, chord progressions~\cite{huang2019music}, or even recipes~\cite{kiddon2016globally}. Future work might also investigate how similar principles could support cases where more than a single end-user and a single model aim to collaborate.\looseness=-1 

% A major future challenge towards progress on collaborative models is that current off-the-shelf deep learning models do not support the semantic inference necessary for CSI interfaces. 
% It is also crucial to note that not every problem benefits from CSI, for example all feature-driven applications such as architecture search and hyperparameter tuning. 
% While CSI models can expose a number of interpretable reasoning steps, they still suffer from similar black-box problems as other neural networks, since the rest of the model remains non-understandable. 
%While black-box explanations in interactive observation tools can yield efficiency increases while improving trust of humans in a machine learning model~\cite{lai2018human}, they can also lead to users trusting the information blindly~\cite{yin2019understanding}. 
%Thus, users retain agency over previously black-box approaches while simultaneously benefiting from the improved efficiency of deep learning models. 

Finally, it is crucial to develop ways to systematically evaluate collaborative interfaces and to investigate the implications of designing algorithmic interactions with humans~\cite{wilks2010close,williams2018toward}. 
While an interpretability-first approach could assist in highlighting fairness and bias issues in data or models~\cite{hughes2018semi, holstein2018improving}, it could also introduce unwanted biases by guiding the user towards what the model has learned~\cite{arnold2018sentiment}. It is thus insufficient to limit the evaluation of a system to measures of efficiency and accuracy. Future work needs to address these shortcomings by developing nuanced evaluation strategies that can detect undesired biases and their effect on end-users. 


%By interacting with the visual interface, the users can avoid unethical output and similarly to prevent factual errors. 
%In first steps towards universally applied CSI models, Google translate recently introduced a semi-collaborative approach to prevent gender-discrimination in translation systems. By treating the gender as a hook, they can present both possible options whenever the gender in a language is ambiguous, for example in Turkish. This approach allows a user to pick the translation they meant, given the wider context and their intrinsic knowledge.

We provide a demo, the code, and the required models for CSI:Summarization at \url{www.c-s-i.ai}.% upon acceptance. 
 

%Furthermore, the use of these models is restricted by available human resources for the tasks they complete, whereas fully autonomous models require less supervision. In many use cases this is a benefit since it forces users of a model to double-check its outputs, but in others it might restrict the scalability. Finally, it is currently not well understood how these models can be formally evaluated without large-scale human studies. 

%We plan to further investigate CSI models in future work to help humans retain the agency over their automated processes and prevent unethical behavior of machine learning models. 

\section*{Acknowledgements}

We would like to thank Michael Behrisch for constructive discussions. This work was funded in
part by the NIH grant 5R01CA204585-02, an AWS Faculty Award and a Google Faculty Award.  

==> Latvaria(IEEEVAST2019) (2)/src/99-notes.tex <==
\newpage
\newpage

\section{Related unrelated work}
\label{sec:notes}
\emph{Notes for papers and random ideas below. A blue checkmark indicates that it was incorporated in the main text.}

\subsection{HCI}
\begin{itemize}
    \item CueFlik describes a tool in which users can define filters for images according to their preferences and can apply these filters on search results~\cite{fogarty2008cueflik}. In clustering, it has been shown that interaction between a model and human experts can lead to better results~\cite{caruana2006meta, cohn2003semi}. \bluecheck
    \item There is a vast literature on the efficient elicitation of user feedback for predictions of machine learning models and incorporating it into the prediction process~\cite{stumpf2009interacting}. \bluecheck
    \item Other models use an interactive system to efficiently develop a rule-based model from the ground up~\cite{oblinger2006augmentation}. \bluecheck
    \item Some recent work aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating} \bluecheck
    \item Kulesza et al. introduce the concept of explanatory debugging that relies on similar bidirectional interactions with a model~\cite{kulesza2010explanatory}. In following work, they provide an argument that explanatory debugging can lead to better personalization and improved mental models~\cite{kulesza2015principles}. \bluecheck
    \item Users who receive explanations about a models rules of behavior are able to better personalize them~\cite{bostandjiev2012tasteweights}. Without such explanations, users fail to develop a mental model of a systems behavior~\cite{lim2009and}. \bluecheck
    \item It is known that explanations should not overwhelm the user. However, many previous approaches take this as the reason to select less complex models~\cite{lacave2002review} or to reduce the feature space of a trained model~\cite{craven1997using, yang1997comparative}. Opposed to this, we propose to develop explanations into the model itself. \bluecheck
    \item Related fields are interactive machine learning and UX for machine learning as UX in the HCI community~\cite{fails2003interactive, amershi2014power,yang2018machine}. While most work concentrates on iterative improvements of models, many findings are applicable to the design process described here. \bluecheck
    \item In computational social science, machine learning is often used as means to an end. Here, the explainability comes from the results itself and not the process and improved models can improve the accuracy of studies~\cite{jordan2015machine}. In computational creativity, machine learning models can be used to facilitate interactions between humans~\cite{siangliulue2016ideahound}. \bluecheck
    \item Collaborative interfaces can introduce unwanted biases~\cite{arnold2018sentiment} \bluecheck
    \item Interaction with the visual metaphor, which resembles the mental model of a user, is also called semantic interaction~\cite{endert2012semantic}. \bluecheck
\end{itemize}

\subsection{AI}
\begin{itemize}
    \item In the 1994 AAAI presidential address, Barbara Grosz argued that the development of ``intelligent, problem-solving partners is an important goal in the science of AI'' and that the capability of applications to collaborate with their users is ``essential''~ \cite{grosz1996collaborative}. \bluecheck
    \item It is increasingly important to consider ethical implications of designing algorithmic interactions with humans~\cite{wilks2010close,williams2018toward}. We base our ethical argument on the framework by D\"orr and Hollnbuchner who discuss ethical challenges in algorithmic journalism~\cite{dorr2017ethical}. In their framework, each user aims to uphold the principles of objectiveness, transparency and accuracy, but is subject to external constraints that sometimes prevents moral action. An algorithm in semi-algorithmic content generation represents one such constraint, since it introduces an additional actor with their own moral guidelines. Typically, the algorithms are treated as relatively autonomous actors with delegated (moral) agency. As such, it is the responsibility of the creator and the user to ensure minimal contradicting behavior. \bluecheck
\end{itemize}

\subsection{Vis}
\begin{itemize}
    \item Interpretation of machine learning models is of particular interest to the visual analytics community. Visual techniques can be applied to explore the behavior of complex models~\cite{zhao2019iforest, strobelt2018lstmvis} and to debug errors~\cite{zhang2019manifold, strobelt2018debugging, krause2017workflow}. \bluecheck
    \item There have been many recent visual analytics approaches to the visualization of increasingly multi-modal input- and output-types. While most interpretability approaches focus on classification~\cite{krause2017workflow}, interactive visualization approaches for text have not converged towards a coherent set of techniques. Text-based problems such as entailment~\cite{liu2019nlize}, QA~\cite{kwon2019retainvis}, and translation~\cite{strobelt2018debugging} have been approached by different visualization strategies. A commonality between them is that all these methods aim to enable interactivity between a user and the model. \bluecheck 
    \item Sacha et al. point out that only few works consider the model development as part of the VA pipeline~\cite{sacha2019vis4ml}. In fact, the visualization of intermediate result has been pointed out as one of the promising future direction for visualization for machine learning~\cite{endert2017state} and has mostly been used to interact with data during time-intensive analysis pipelines instead of as explicitly modeled part of the interaction~\cite{stolper2014progressive}. There has also been a distinct lack of visual tools designed for non-experts that are not used as teaching tools~\cite{hohman2018visual}. \bluecheck
    \item 
\end{itemize}

\subsection{FAT*}
\begin{itemize}
    \item Recent work found that explanations or simple information about a classifier can raise the efficiency and trust of humans in a machine learning model~\cite{lai2018human}, but can also lead to users trusting the information over the observed model output~\cite{yin2019understanding}. This shows that explainability can to some degree mediate in the agency vs efficiency trade-off. We argue that interactive explanations and predictions help help even more. \bluecheck
    \item Evaluation of explainability methods is complex and simple A/B tests are insufficient to measure the impact that types of explanations have on users~\cite{lage2019evaluation}. Sometimes, methods for interpretability even pick up on spurious correlations in inputs and ignore the model that they aim to analyze~\cite{SanityNIPS2018, 2017arXiv171100867K}. Moreover, since explanations are typically task-specific, findings rarely generalize and some explanations do not scale well due to visual overload~\cite{poursabzi2018manipulating}. To address this problem, the effectiveness of different methods needs to be carefully evaluated in real-world or proxy tasks~\cite{doshi2018considerations}. Some recent work has tried to automated the iterative development and testing-process by including user-studies within the development cycles~\cite{lage2018human}. \bluecheck
    \item Lipton describes two necessary properties of interpretable models - transparency in derivation and post-hoc interpretability for non-experts~\cite{lipton2016mythos}. Following these properties, the method for deriving values of hooks should be easily understandable and their values should make sense even to non-expert users. \bluecheck
    \item The UX design of machine learning models is in its early stages and we urgently need to develop that can expose fairness and bias issues in underlying data and models~\cite{holstein2018improving}. By visually exposing intermediate decisions to the user, even without interaction, this could lead to an earlier detection of these issues. \bluecheck
    \item In addition to conditional generation tasks, our framework can be applied to problems that can be categorized as creative AI, where models help users create stories~\cite{fan2018hierarchical}, chord progressions~\cite{huang2019music}, or even recipes~\cite{kiddon2016globally}. Now imagine that, since most people who write recipes agree that kale is vastly inferior to spinach, a model has learned this underlying information and always includes spinach instead of kale in recipes. An analogous argument can be made for the development of characters in story, who, following the popular story corpora, would be mainly white and male. However, by explicitly modeling the character (or vegetable) choices as a latent variable, a user could actively prevent this discrimination from happening without having to give up the assistive technology. We note that, as all technology is evil, this method can theoretically also be used to actively discriminate. \bluecheck
\end{itemize}

\section{Technical background}

\subsection{Applying the framework to analyze a technical paper}
\begin{itemize}
    \item I was thinking we could use section one to identify potential interactions in \cite{wiseman2018learning}
    \item Points to visualization challenge: How to visualize abstract clusters during text-generation
\end{itemize}

\section{Jeff Herr paper}

 \cite{Heer1844} -- Notes are in-depth.
\begin{itemize}
    \item Current work on automation does not consider the design space in which computational assistance augments and enriches people's intellectual work. 
    \item His use-cases:
    \begin{itemize}
        \item data wrangling $\leftarrow$ We don't 
        \item exploration $\leftarrow$ ?
        \item machine translation $\leftarrow$ Interaction is forward only. Subtle difference, we'll have to make it very clear. It is also non-neural translation and his approach will require changing neural models
    \end{itemize}
    \item intelligence augmentation: Using computers to extend people's ability to process information and reason about problems --- another connection to LatVarIA?
    \item 
    \begin{itemize}
        \item Automation can mislead due to bias
        \item humans can overly rely on predictions, potential loss of expertise/accurate supervision
        \item Humans need to supervise to prevent discrimination and ensure cultural appropriateness
    \end{itemize}
    \item His question: How can we effectively integrate automated reasoning into user-centered interactive systems $\rightarrow$ This reasoning is too narrow. We don't want to simply integrate suggestions, we want true collaboration
    \item His feedback mechanism (our backwards step) is purely focused on improving the model 
    \item Examples: Spell checkers and predictive typing. They increase efficiency - do they also increase efficacy? They do not explain their predictions in most cases and can misguide users to write differently from what they originally intended (Ken's research)
    \item Predictive systems can lead humans to consider alternatives that they would otherwise not have considered $\rightarrow$ Pao's research might be relevant about exploring design spaces in ideation. He also found that suggesting systems that promote diversity can lead to a better coverage of the design space
    \item $\rightarrow$ He has the same goal of codesigning interfaces and algorithms, but only suggests a more limited approach. In this, there are predictions and feedback. Nothing else (notable difference is the coverage in translation, which is not applicable to neural models)
    \item By exploration, he means exploration of data, not the model
    \item Open question: How might people not only work with algorithms via an a priori shared representation, but construct new representations in a data-driven manner? How might shared representations help promote interpretability?
\end{itemize}

\subsection{Model and Process Papers}

VIS4ML proposes an ontology for VA-assisted machine learning~\cite{sacha2019vis4ml}. \bluecheck

State-of-the-art-reports and classification of existing works on integrating machine learning into visual analytics (with process/pipeline figures)~\cite{endert2017state, liu2017towards, lu2017state}. \bluecheck % need to cite later again

Survey/taxonomy paper zu Visual Analytics und Deep Learning~\cite{hohman2018visual} (discusses interpretability, explainability, comparison, debugging and improving models, audiences for it, etc..  also good starting point to find more literature) \bluecheck

An analysis of machine-and human-analytics in classification~\cite{tam2017analysis} \bluecheck

\subsection{VA and Sequence Models}
% Strobelt et al.~\cite{strobelt2019s, strobelt2018debugging, strobelt2018lstmvis}
Islam et al. presents an approach which helps to visualize the internal reasoning of sequence learning models on audio data~\cite{islam2018gray}.


\section{Directly interpretable model architectures from Grant}

Along with model improvement, a target of some recently developed methods is the extension of neural models to allow for easier interpretation~\cite{caruana2015intelligible}.  In natural language processing, a popular
technique has been to use an attention-mechanism to allow the model to
focus in on a particular aspect of the input. Attention is used for
soft alignment in machine translation~\cite{Bahdanau2015}, to identify
important aspects of an image for
captioning~\cite{DBLP:conf/icml/XuBKCCSZB15}, to find important
aspects of a document for an extraction task~\cite{HermannKGEKSB15},
along with many other relevant applications. We discuss attention and
related techniques in more detail below. An important aspect of our proposed work is the direct manipulation of these user-friendly components. In a preliminary approach, Lee et
al.~\cite{lee2017interactive} present a tool that can visualize the attention in a machine translation task and find that the alignment between source and target language is often ambiguous. While their tool lets a user investigate a local fix, it does not provide a feedback mechanism to improve the model based on the interaction.


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> src/03-related.tex <==
%\section{Related Work}

%Our framework combines insights from the fields of artificial intelligence, human-computer interaction, and visual analytics, some of which have a long-standing history. In the 1994 AAAI presidential address, Barbara Grosz argued that the development of ``intelligent, problem-solving partners is an important goal in the science of AI'' and that the capability of applications to collaborate with their users is ``essential''~\cite{grosz1996collaborative}. This call is further reflected in one of Horvitz' principles for mixed-initiative user interfaces~\cite{horvitz1999principles} and the more recent guidelines for human-AI interaction~\cite{amershi2019guidelines} which call for ``mechanisms for efficient agent-user collaboration to refine results.'' In a similar argument, Jeffrey Herr argues that work on automation does not consider the design space in which computational assistance augments and enriches people's intellectual work~\cite{Heer1844}. Opposed to our framework, these guidelines do not consider incorporating interactive facets into the model itself to enable efficient interaction.
%There also exist a vast literature on the efficient elicitation of user feedback for predictions of machine learning models~\cite{stumpf2009interacting} and the UX for machine learning~\cite{fails2003interactive, amershi2014power,yang2018machine}. While most related work concentrates on iterative model improvements, many findings can be formulated in the context of the interactive collaboration framework. 
%We further note similarities to the concept of explanatory debugging by Kulesza et al. that relies on interactions with a model~\cite{kulesza2010explanatory}, and which they find can lead to better personalization and improved mental models~\cite{kulesza2015principles}.

%Another important aspect of our work is that the interpretable parts of a model can act as explanations for rules of behavior that models learn. This kind of explanation has been shown to improve model personalization~\cite{bostandjiev2012tasteweights} and explainability~\cite{caruana2015intelligible}, while failing to provide explanations can inhibit development of mental models in users~\cite{lim2009and}. It is also known that explanations should not overwhelm a user and many previous approaches thus select less complex models~\cite{lacave2002review} or aim to reduce the feature space of a trained model~\cite{craven1997using, yang1997comparative}. Opposed to this, our proposed framework is agnostic to the model complexity, since the explanations are built into the model.

%Sacha et al. point out that only few works consider the model development as part of the visual analytics pipeline~\cite{sacha2019vis4ml}. In fact, the visualization of intermediate result has been pointed out as one of the promising future direction for visualization for machine learning~\cite{endert2017state} and has mostly been used to interact with data during time-intensive analysis pipelines instead of as explicitly modeled part of the interaction~\cite{stolper2014progressive}. There has also been a distinct lack of visual tools designed for non-experts that are not used as teaching tools~\cite{hohman2018visual}.

%\subsection{The Visualization Techniques}

%The development of methods for interactive, but not collaborative, visual interfaces has been an active field of research, as summarized in recent review papers~\cite{endert2017state, liu2017towards, lu2017state, hohman2018visual}.
%The visual approaches to integrate an expert's domain knowledge range from user-guided instance and feature selection~\cite{}, interactive parameter configuration~\cite{}, to active~\cite{holzinger2016interactive,cohn1996active}, and augmented-based learning~\cite{oblinger2006augmentation}.

%The visualization techniques relevant to our goal aim to understand how blackbox models work, how they perform under varying conditions, and how to debug and improve them.
%A step towards better model understanding is Google's \textit{What-If} tool~\cite{whatif}. Such counterfactual explanations~\cite{wachter2017counterfactual} allow to investigate changes in the outcome of a model for different inputs, thereby increasing trust and interpretability.
%This is especially of interest when models get increasingly complex, as it appears for deep learning approaches. One frequent proposal is to visually explore model internals and behavior to better understand them, as has been done for recurrent networks under varying conditions~\cite{strobelt2018lstmvis}. 
%Other methods focus more on debugging errors~\cite{zhang2019manifold, strobelt2018debugging, krause2017workflow} and only visualizing the necessary parts to find and explain them, instead of giving in-depth insights into hidden states.

%While many interpretability approaches concern classification problems~\cite{krause2017workflow,tam2017analysis} and can be applied to multi-modal input and output types, recent proposals for text have not yet converged towards a single set of techniques. Especially text-based problems such as entailment~\cite{liu2019nlize}, question answering~\cite{kwon2019retainvis}, and translation~\cite{strobelt2018debugging} have been approached by different visualization strategies. Following their insights that high-dimensional vectors are not interpretable, our use-cases do not include any visualizations of the hidden states. Instead, we focus the visualization efforts on those aspects of a model that can be readily understood by non-expert users. 

%We further identify similarities between collaborative approaches and the concept of models as a team member. Here, studies have shown that interactive models can improve the accuracy of studies~\cite{jordan2015machine}, facilitate interactions between multiple team members~\cite{siangliulue2016ideahound}, and improve the models themselves~\cite{fogarty2008cueflik, caruana2006meta, cohn2003semi}. Some recent work even aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating}. Thus, designing the model as a team member rather than a static resource can vastly improve outcomes. 

% \subsection{The Visualization Techniques}
% % Debugging/Analysis
% In this section, we contextualize the methods we applied to develop our use-cases within the related work and present alternative analysis and visualization approaches. A more general overview on combining machine learning with visual interfaces can be found in recent review papers~\cite{endert2017state, liu2017towards, lu2017state, hohman2018visual}.

% Interpretation of machine learning models is of particular interest to the visual analytics community, since visual techniques allow to better explore the behavior of complex models~\cite{zhao2019iforest, strobelt2018lstmvis} and to debug errors~\cite{zhang2019manifold, strobelt2018debugging, krause2017workflow}.
% Visual analytics can be applied to increasingly multi-modal input- and output-types. While many interpretability approaches focus on classification problems~\cite{krause2017workflow,tam2017analysis}, recent visual analysis means for text have not yet converged towards a single set of techniques. Especially text-based problems such as entailment~\cite{liu2019nlize}, question answering~\cite{kwon2019retainvis}, and translation~\cite{strobelt2018debugging} have been approached by different visualization strategies. 
% Following insights\rk{which insights?} from these papers, our use-cases do not include any visualizations of the high-dimensional hidden states. Instead, we focus the visualization efforts on those aspects of a model that can be readily understood by non-expert users.

% % Means to end
%\rk{I dont understand this part}
% Other inspirations of our presented use-cases originate in research on interactivity between user and model in computational social science. Here, the explainability often comes from the results itself instead of the process, and improved models can improve the accuracy of studies~\cite{jordan2015machine}, facilitate interactions between multiple team members~\cite{siangliulue2016ideahound}, and improve the models themselves~\cite{fogarty2008cueflik, caruana2006meta, cohn2003semi}. Some recent work even aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating}. Thus, designing the model as a team member rather than a static resource can vastly improve outcomes. 

% % Active Learning
% We differentiate our approach from work on interactive systems that aim to train models from the ground up, for example using different active learning techniques~\cite{holzinger2016interactive,cohn1996active} or systems that can be used to efficiently develop rule-based models from the ground up~\cite{oblinger2006augmentation}. 

==> src/04-captioning.tex <==
\section{Use Case 1: A Collaborative Captioning Model}
\label{sec:uc1}

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth, draft]{"figs/LSTM_S2S_Latvaria_Levers"}
    \caption{\sg{Screenshot todo} Interface overview for captioning. }
    \label{fig:cap-overview}
\end{figure}

We choose image captioning as the first collaborative interface. Image captioning describes the problem of generating a description of an image that accurately captures its content. From the machine learning side, this problem is typically addressed with a sequence-to-sequence model with attention, which represents which part of an image the currently generated word focused on~\cite{DBLP:conf/icml/XuBKCCSZB15}.
Imagine a user Anne, who wants to use an interface, powered by a captioning model, to help her generate captions. With an unmodified forward model, we can design an interface where Anne can upload an image and the model suggests a caption. However, if Anne does not like the caption, she needs to post-edit the suggestion to her liking. Moreover, if the model focuses on the wrong object in the image, Anne has to write the entire caption from scratch. There is also no visual indication if a caption captures all the information available in the image. 

%use-case ideas: user wants to create captions, loads image, runs model, reads result, not satisfactory, adds and rearranges detected objects in the image, reruns model, better output, one wrong part, user makes corrections (also corrects attention), models shows most suitable input to achieve that, user again edits input, runs model, is satisfied with output.

We can address some of these issues without a modified model. Following insights from mixed-initiative writing assistants~\cite{babaian2002writer}, the interface should enable Anne to request model-input. For example, she should be able to write one sentence and have the model generate the second. Since this does not require any feedback towards the model, we can use a a constrained prediction similar to that in Seq2Seq-Vis~\cite{strobelt2019s}.

However, this interface does not prevent the model from focusing on objects that Anne might not want. For this, we need to be able to constrain the latent variable. A natural approach for the semantic interaction is to allow Anne to select objects in the input which tells the model what to generate. 
For this use case, we redefine the attention as a latent variable, similar to the approach by Deng et al.~\cite{deng2018latent}. This enables the forward semantic interaction through object selection. 

In the backwards interaction, Anne may want to know what part of the image she hasn't described yet. Since we have defined the attention over objects in the image, we can aggregate the attention over the entire collaboratively written caption\footnote{While the standard attention can be easily explained and visualized, the weights without a hook network do not directly correspond to explanations and are often ambiguous~\cite{lee2017interactive, Jain2019attention}.}. 


\subsection{Visual Design}


Notes:
- visual design considerations: 

- visual interface shows input-model-output. user can explore how input objects is connected to output objects.

- reduce visual clutter with edge bundling through proxies, emphasize objects in focus through highlighting/color coding.

- keep overview by hierarchical aggregation of input and output objects. words to sentences. (maybe more important for second use case)

- user can emphasize (but not enforce) objects/regions of interest in the input image, and output caption. - model takes this into account - collaboration.

- further user actions: add/delete/edit object regions in the input, edit captioning in the output - visual interface shows most suitable matches to achieve this output in the input space.


==> src/99-notes.tex <==
\newpage
\newpage

\section{Related unrelated work}
\label{sec:notes}
\emph{Notes for papers and random ideas below. A blue checkmark indicates that it was incorporated in the main text.}

\subsection{HCI}
\begin{itemize}
    \item CueFlik describes a tool in which users can define filters for images according to their preferences and can apply these filters on search results~\cite{fogarty2008cueflik}. In clustering, it has been shown that interaction between a model and human experts can lead to better results~\cite{caruana2006meta, cohn2003semi}. \bluecheck
    \item There is a vast literature on the efficient elicitation of user feedback for predictions of machine learning models and incorporating it into the prediction process~\cite{stumpf2009interacting}. \bluecheck
    \item Other models use an interactive system to efficiently develop a rule-based model from the ground up~\cite{oblinger2006augmentation}. \bluecheck
    \item Some recent work aimed to generate text that describes an image such that a human can understand the prediction process of a model~\cite{hendricks2016generating} \bluecheck
    \item Kulesza et al. introduce the concept of explanatory debugging that relies on similar bidirectional interactions with a model~\cite{kulesza2010explanatory}. In following work, they provide an argument that explanatory debugging can lead to better personalization and improved mental models~\cite{kulesza2015principles}. \bluecheck
    \item Users who receive explanations about a models rules of behavior are able to better personalize them~\cite{bostandjiev2012tasteweights}. Without such explanations, users fail to develop a mental model of a systems behavior~\cite{lim2009and}. \bluecheck
    \item It is known that explanations should not overwhelm the user. However, many previous approaches take this as the reason to select less complex models~\cite{lacave2002review} or to reduce the feature space of a trained model~\cite{craven1997using, yang1997comparative}. Opposed to this, we propose to develop explanations into the model itself. \bluecheck
    \item Related fields are interactive machine learning and UX for machine learning as UX in the HCI community~\cite{fails2003interactive, amershi2014power,yang2018machine}. While most work concentrates on iterative improvements of models, many findings are applicable to the design process described here. \bluecheck
    \item In computational social science, machine learning is often used as means to an end. Here, the explainability comes from the results itself and not the process and improved models can improve the accuracy of studies~\cite{jordan2015machine}. In computational creativity, machine learning models can be used to facilitate interactions between humans~\cite{siangliulue2016ideahound}. \bluecheck
    \item Collaborative interfaces can introduce unwanted biases~\cite{arnold2018sentiment} \bluecheck
    \item Interaction with the visual metaphor, which resembles the mental model of a user, is also called semantic interaction~\cite{endert2012semantic}. \bluecheck
\end{itemize}

\subsection{AI}
\begin{itemize}
    \item In the 1994 AAAI presidential address, Barbara Grosz argued that the development of ``intelligent, problem-solving partners is an important goal in the science of AI'' and that the capability of applications to collaborate with their users is ``essential''~ \cite{grosz1996collaborative}. \bluecheck
    \item It is increasingly important to consider ethical implications of designing algorithmic interactions with humans~\cite{wilks2010close,williams2018toward}. We base our ethical argument on the framework by D\"orr and Hollnbuchner who discuss ethical challenges in algorithmic journalism~\cite{dorr2017ethical}. In their framework, each user aims to uphold the principles of objectiveness, transparency and accuracy, but is subject to external constraints that sometimes prevents moral action. An algorithm in semi-algorithmic content generation represents one such constraint, since it introduces an additional actor with their own moral guidelines. Typically, the algorithms are treated as relatively autonomous actors with delegated (moral) agency. As such, it is the responsibility of the creator and the user to ensure minimal contradicting behavior. \bluecheck
\end{itemize}

\subsection{Vis}
\begin{itemize}
    \item Interpretation of machine learning models is of particular interest to the visual analytics community. Visual techniques can be applied to explore the behavior of complex models~\cite{zhao2019iforest, strobelt2018lstmvis} and to debug errors~\cite{zhang2019manifold, strobelt2018debugging, krause2017workflow}. \bluecheck
    \item There have been many recent visual analytics approaches to the visualization of increasingly multi-modal input- and output-types. While most interpretability approaches focus on classification~\cite{krause2017workflow}, interactive visualization approaches for text have not converged towards a coherent set of techniques. Text-based problems such as entailment~\cite{liu2019nlize}, QA~\cite{kwon2019retainvis}, and translation~\cite{strobelt2018debugging} have been approached by different visualization strategies. A commonality between them is that all these methods aim to enable interactivity between a user and the model. \bluecheck 
    \item Sacha et al. point out that only few works consider the model development as part of the VA pipeline~\cite{sacha2019vis4ml}. In fact, the visualization of intermediate result has been pointed out as one of the promising future direction for visualization for machine learning~\cite{endert2017state} and has mostly been used to interact with data during time-intensive analysis pipelines instead of as explicitly modeled part of the interaction~\cite{stolper2014progressive}. There has also been a distinct lack of visual tools designed for non-experts that are not used as teaching tools~\cite{hohman2018visual}. \bluecheck
    \item 
\end{itemize}

\subsection{FAT*}
\begin{itemize}
    \item Recent work found that explanations or simple information about a classifier can raise the efficiency and trust of humans in a machine learning model~\cite{lai2018human}, but can also lead to users trusting the information over the observed model output~\cite{yin2019understanding}. This shows that explainability can to some degree mediate in the agency vs efficiency trade-off. We argue that interactive explanations and predictions help help even more. \bluecheck
    \item Evaluation of explainability methods is complex and simple A/B tests are insufficient to measure the impact that types of explanations have on users~\cite{lage2019evaluation}. Sometimes, methods for interpretability even pick up on spurious correlations in inputs and ignore the model that they aim to analyze~\cite{SanityNIPS2018, 2017arXiv171100867K}. Moreover, since explanations are typically task-specific, findings rarely generalize and some explanations do not scale well due to visual overload~\cite{poursabzi2018manipulating}. To address this problem, the effectiveness of different methods needs to be carefully evaluated in real-world or proxy tasks~\cite{doshi2018considerations}. Some recent work has tried to automated the iterative development and testing-process by including user-studies within the development cycles~\cite{lage2018human}. \bluecheck
    \item Lipton describes two necessary properties of interpretable models - transparency in derivation and post-hoc interpretability for non-experts~\cite{lipton2016mythos}. Following these properties, the method for deriving values of hooks should be easily understandable and their values should make sense even to non-expert users. \bluecheck
    \item The UX design of machine learning models is in its early stages and we urgently need to develop that can expose fairness and bias issues in underlying data and models~\cite{holstein2018improving}. By visually exposing intermediate decisions to the user, even without interaction, this could lead to an earlier detection of these issues. \bluecheck
    \item In addition to conditional generation tasks, our framework can be applied to problems that can be categorized as creative AI, where models help users create stories~\cite{fan2018hierarchical}, chord progressions~\cite{huang2019music}, or even recipes~\cite{kiddon2016globally}. Now imagine that, since most people who write recipes agree that kale is vastly inferior to spinach, a model has learned this underlying information and always includes spinach instead of kale in recipes. An analogous argument can be made for the development of characters in story, who, following the popular story corpora, would be mainly white and male. However, by explicitly modeling the character (or vegetable) choices as a latent variable, a user could actively prevent this discrimination from happening without having to give up the assistive technology. We note that, as all technology is evil, this method can theoretically also be used to actively discriminate. \bluecheck
\end{itemize}

\section{Technical background}

\subsection{Applying the framework to analyze a technical paper}
\begin{itemize}
    \item I was thinking we could use section one to identify potential interactions in \cite{wiseman2018learning}
    \item Points to visualization challenge: How to visualize abstract clusters during text-generation
\end{itemize}

\section{Jeff Herr paper}

 \cite{Heer1844} -- Notes are in-depth.
\begin{itemize}
    \item Current work on automation does not consider the design space in which computational assistance augments and enriches people's intellectual work. 
    \item His use-cases:
    \begin{itemize}
        \item data wrangling $\leftarrow$ We don't 
        \item exploration $\leftarrow$ ?
        \item machine translation $\leftarrow$ Interaction is forward only. Subtle difference, we'll have to make it very clear. It is also non-neural translation and his approach will require changing neural models
    \end{itemize}
    \item intelligence augmentation: Using computers to extend people's ability to process information and reason about problems --- another connection to LatVarIA?
    \item 
    \begin{itemize}
        \item Automation can mislead due to bias
        \item humans can overly rely on predictions, potential loss of expertise/accurate supervision
        \item Humans need to supervise to prevent discrimination and ensure cultural appropriateness
    \end{itemize}
    \item His question: How can we effectively integrate automated reasoning into user-centered interactive systems $\rightarrow$ This reasoning is too narrow. We don't want to simply integrate suggestions, we want true collaboration
    \item His feedback mechanism (our backwards step) is purely focused on improving the model 
    \item Examples: Spell checkers and predictive typing. They increase efficiency - do they also increase efficacy? They do not explain their predictions in most cases and can misguide users to write differently from what they originally intended (Ken's research)
    \item Predictive systems can lead humans to consider alternatives that they would otherwise not have considered $\rightarrow$ Pao's research might be relevant about exploring design spaces in ideation. He also found that suggesting systems that promote diversity can lead to a better coverage of the design space
    \item $\rightarrow$ He has the same goal of codesigning interfaces and algorithms, but only suggests a more limited approach. In this, there are predictions and feedback. Nothing else (notable difference is the coverage in translation, which is not applicable to neural models)
    \item By exploration, he means exploration of data, not the model
    \item Open question: How might people not only work with algorithms via an a priori shared representation, but construct new representations in a data-driven manner? How might shared representations help promote interpretability?
\end{itemize}

\subsection{Model and Process Papers}

VIS4ML proposes an ontology for VA-assisted machine learning~\cite{sacha2019vis4ml}. \bluecheck

State-of-the-art-reports and classification of existing works on integrating machine learning into visual analytics (with process/pipeline figures)~\cite{endert2017state, liu2017towards, lu2017state}. \bluecheck % need to cite later again

Survey/taxonomy paper zu Visual Analytics und Deep Learning~\cite{hohman2018visual} (discusses interpretability, explainability, comparison, debugging and improving models, audiences for it, etc..  also good starting point to find more literature) \bluecheck

An analysis of machine-and human-analytics in classification~\cite{tam2017analysis} \bluecheck

\subsection{VA and Sequence Models}
% Strobelt et al.~\cite{strobelt2019s, strobelt2018debugging, strobelt2018lstmvis}
Islam et al. presents an approach which helps to visualize the internal reasoning of sequence learning models on audio data~\cite{islam2018gray}.


\section{Directly interpretable model architectures from Grant}

Along with model improvement, a target of some recently developed methods is the extension of neural models to allow for easier interpretation~\cite{caruana2015intelligible}.  In natural language processing, a popular
technique has been to use an attention-mechanism to allow the model to
focus in on a particular aspect of the input. Attention is used for
soft alignment in machine translation~\cite{Bahdanau2015}, to identify
important aspects of an image for
captioning~\cite{DBLP:conf/icml/XuBKCCSZB15}, to find important
aspects of a document for an extraction task~\cite{HermannKGEKSB15},
along with many other relevant applications. We discuss attention and
related techniques in more detail below. An important aspect of our proposed work is the direct manipulation of these user-friendly components. In a preliminary approach, Lee et
al.~\cite{lee2017interactive} present a tool that can visualize the attention in a machine translation task and find that the alignment between source and target language is often ambiguous. While their tool lets a user investigate a local fix, it does not provide a feedback mechanism to improve the model based on the interaction.

